A Semi-Algebraic Framework for Verification and Synthesis of Control Barrier Functions

Safety is a critical property for control systems in medicine, transportation, manufacturing, and other applications, and can be defined as ensuring positive invariance of a predefined safe set. This paper investigates the problems of verifying positive invariance of a semi-algebraic set as well as synthesizing sets that can be made positive invariant through Control Barrier Function (CBF)-based control. The key to our approach consists of mapping conditions for positive invariance to sum-of-squares constraints via the Positivstellensatz from real algebraic geometry. Based on these conditions, we propose a framework for verifying safety of CBF-based control including single CBFs, high-order CBFs, multi-CBFs, and systems with trigonometric dynamics and actuation constraints. In the area of synthesis, we propose algorithms for constructing CBFs, namely, an alternating-descent approach and a local CBF approach. We evaluate our approach through case studies on quadrotor UAV and power converter test systems.

==> First-revision/Response-document/Reviewer_10_comments.tex <==
\begin{center}
\textbf{Reviewer 10 Comments and Response}
\end{center}


\begin{itemize}
\item \underline{Initial Comments of Reviewer 10:} This paper studied the verification and synthesis of control barrier
functions and controlled positive invariant sets. Author showed that
verifying that a semi-algebraic set is controlled positive invariant
for a system with polynomial dynamics is equivalent to the
non-existence of a solution to a system of polynomial equations and
inequalities. The author then proved that controlled positive
invariance is equivalent to a sum-of-squares optimization problem via
the Positivstellensatz. The author generalized this approach to systems
with trigonometric dynamics, actuation constraints, and Lagrangian
dynamics. The following problems can be clarified. \\

\item \underline{Response to Initial Comments of Reviewer 10:} We thank the reviewer for taking the time to provide detailed comments. In what follows, we reproduce each comment, respond, and describe how the comment has been incorporated into the revised manuscript.\\



\item \underline{Comment \#1 of Reviewer 10:} The main contribution and challenge encountered in this paper are not
clear. what are the main difficulties for the investigation? And what
is your main contribution? Please clarify.\\

\item \underline{Response to Comment \#1 of Reviewer 10:} The main contributions of the paper are related to verification and synthesis of semi-algebraic invariant sets for nonlinear control systems. In the area of verification, we study the problem of determining whether a given semi-algebraic set can be rendered positive invariant through control. While tangential conditions of positive invariance are available in the literature, computational approaches for verifying those conditions have been less-studied. We propose a framework that leverages theorems of alternatives, especially the Positivstellensatz from real algebraic geometry and Farkas Lemma from linear algebra, to formulate sum-of-squares programs that can be used to compute safety certificates. \\

In the area of synthesis, we propose two algorithms for constructing positive invariant sets. The first algorithm uses an alternating descent method based on the SOS programs that we derived for verification. The second algorithm constructs one or more CBFs that are valid in a local neighborhood of a safe equilibrium points. \\ 

\item \underline{Comment \#2 of Reviewer 10:} The abbreviation should be the full name when it first appears in
this paper.\\

\item \underline{Response to Comment \#2 of Reviewer 10:} We have used made sure to introduce abbreviations by the full name in the first place they appear.\\


\item \underline{Comment \#3 of Reviewer 10:} The analysis of the simulation part is insufficient, and it is
suggested that the author improve it. The simulation result graph is
missing, the author should make a supplement and add a description so
that the framework proposed in this paper can be further verified.\\

\item \underline{Response to Comment \#3 of Reviewer 10:} We have extended the simulation study to consider a nontrivial example of a linearized quadrotor with actuation constraints. We have provided additional details on the simulation setup and plots to illustrate the results.\\

\item \underline{Comment \#4 of Reviewer 10:} Some lemmas lack corresponding proofs. In addition, it is recommended
that the author add 1-2 Remarks to improve readability for readers.
Compared to existing work, in order to highlight the advantages of the
paper.\\

\item \underline{Response to Comment \#4 of Reviewer 10:} We have included all proofs in the paper, with some proofs in the appendices for clarity of presentation. We have added remarks and examples throughout the papers to improve understanding.\\

\item \underline{Comment \#5 of Reviewer 10:} Before submitting a final manuscript, the author should check the
paper carefully and correct the grammar errors. \\

\item \underline{Response to Comment \#5 of Reviewer 10:} We have proofread the paper and corrected grammar and other typos.

\end{itemize}

==> First-revision/Response-document/Reviewer_15_comments.tex <==
\begin{center}
\textbf{Reviewer 15 Comments and Response}
\end{center}


\begin{itemize}
\item \underline{Initial Comments of Reviewer 15:} For the control Barrier functions (CBFs) related method, how to find a
valid CBF is a critical and challenging problem. 
In this paper, the verification and synthesis of the CBFs are
investigated, where the topic of the research is interesting and
meaningful. In my opinion, this paper deserves to be published as long
as the results are correct. \\

\item \underline{Response to Initial Comments of Reviewer 15:} We thank the reviewer for taking the time to provide detailed comments. In what follows, we reproduce each comment, respond, and describe how the comment has been incorporated into the revised manuscript.\\

\item \underline{Comment \#1 of Reviewer 15:} It should be noted that the actual systems require many control
objectives such as tracking, stability, and safety constraint. In other
words, in addition to security requirements, the most fundamental
stability and tracking difficulties must also be addressed, yet only
security constraints can be handled by the controller in this study. \\

\item \underline{Response to Comment \#1 of Reviewer 15:} The reviewer is correct that stability and tracking are not addressed in the paper. Joint verification of safety and stability, such as through Control Barrier-Lyapunov Functions, are a direction of future study that we will explore.\\

\item \underline{Comment \#2 of Reviewer 15:} On the other hand, certain examples are suggested to be included in
the content to help the reader understand the meaning of the theorem
and definition. \\

\item \underline{Response to Comment \#2 of Reviewer 15:} We thank the reviewer for the comment. We have revised the paper to add examples throughout the technical sections to improve the understanding of the reader.

%\item \underline{Response to Comment \#2 of Reviewer 15:}

\end{itemize}

==> First-revision/Response-document/Reviewer_1_comments.tex <==
\begin{center}
\textbf{Reviewer 1 Comments and Response}
\end{center}
~
\begin{itemize}
\item \underline{Initial Comments of Reviewer 1:} In this paper, the verification of candidate polynomial control barrier functions is addressed for classes of polynomial, nonlinear dynamical systems via various forms of sum-of-squares optimization problems. The authors further propose several iterative algorithms for synthesizing a valid CBF offline, though no numerical or experimental validation of this second contribution is offered.\\

While the results are generally interesting, we have identified some major oversights and/or omissions that need to be addressed.\\

\item \underline{Response to Initial Comments of Reviewer 1:} We thank the reviewer for taking the time to provide detailed comments. In what follows, we reproduce each comment, respond, and describe how the comment has been incorporated into the revised manuscript.\\

\item \underline{Comment \#1 of Reviewer 1:}
If the technical results of the paper rely on Nagumo’s Theorem for set invariance then the necessary conditions need to be met: namely, existence and uniqueness of solutions and $db/dx \neq 0$ for all x on the boundary of the set (see below for an example that demonstrates why this is necessary). If this does not prohibit a discontinuous control input, then this needs to be justified clearly. Further care ought to be taken when referring to the function b as a CBF when it has not been shown to meet the definition of a CBF as defined by Def. 2.\\

\item \underline{Response to Comment \#1 of Reviewer 1:} We thank the reviewer for this helpful comment. We have significantly revised the manuscript to use the correct version of Nagumo's Theorem. In particular, we assume that, if the safe region is of the form $$\mathcal{C} = \{x : b_{i}(x) \geq 0, i=1,\ldots,N\}$$ for some functions $b_{1},\ldots,b_{N}$, then for all $x \in \mathcal{C}$, then there exists $z$ satisfying $\frac{\partial b_{i}}{\partial x}z + b_{i}(x) > 0$ for all $i=1,\ldots,N$. Furthermore when the b's are polynomial, we present an approach for verifying that this condition is satisfied. This assumption is stated explicitly at the beginning of Section IV of the revised manuscript.\\

With respect to existence and uniqueness of solutions, we modify our definition of positive invariance to point out that the system remains in the set $\mathcal{C}$ over the time interval when the solution is defined. Moreover, we point out that, when the safe region is compact and the dynamics are polynomial (and hence locally Lipschitz), a unique solution exists for all time $t$.\\

Finally, in order to address discontinuities, we present two safety problems that are considered separately in the paper. The first class of safety properties relates to \emph{viability}. We say that a set $\mathcal{C}$ is viable for a dynamical system $\dot{x}(t) = f(x(t)) + g(x(t))u(t)$ if, for any $x \in \partial \mathcal{C}$, there exists a $u$ satisfying the conditions of Nagumo's Theorem, i.e., $(f(x) + g(x)u) \in \mathcal{T}_{\mathcal{C}}(x)$, where $\mathcal{T}_{\mathcal{C}}(x)$ denotes the tangent cone to $\mathcal{C}$ at $x$. The second class of safety properties is \emph{feedback controlled positive invariance}. This safety condition implies that there is a continuous control policy $\mu: \mathcal{C} \rightarrow \mathcal{U}$ such that $\mathcal{C}$ is positive invariant under the dynamics $\dot{x}(t) = f(x(t)) + g(x(t))u(t)$.\\

%, and we verify that the system is viable in the standard sense \textbf{*refs}. The second class of safety properties is \emph{feedback controlled positive invariance}. For this class, we prove sufficient conditions for the existence of a continuous control that guarantees safety.\\

%for all $x \in \mathcal{C}_{i}$, there exists $z$ satisfying $\frac{\partial b_{ij}}{\partial x}z + b_{ij}(x) > 0$ for all $j=1,\ldots,r_{i}$.

\item \underline{Comment \#2 of Reviewer 1:} In addition, if it is truly both sufficient and necessary for candidate barrier functions to be SOS rather than simply non-negative polynomials, then this needs to be clearly explained. In general, Section 3 needs significant improvement with regard to both clarity of presentation and relation to CBF verification.\\

\item \underline{Response to Comment \#2 of Reviewer 1:} Under our approach, it is neither necessary nor sufficient for candidate barrier functions to be SOS. We have completely reorganized the sections on safety definition and verification in the revised manuscript. In the revised manuscript, we state clearly that our goal is to verify two safety properties of a given set: viability and feedback controlled positive invariance. We present CBF-based control as a special case  and derive conditions for existence of CBF-based controllers. We have improved the presentation by moving proofs to an appendix and adding examples to illustrate our results.\\

\item \underline{Comment \#3 of Reviewer 1:} It is further concerning that the only demonstration of the many proposed methods contained in the paper is a simplistic example that offers no convincing evidence. Many claims were made throughout the paper as to how the proposed methods improved upon the state-of-the-art, so comparative examples are required to demonstrate how this is true. In addition, a demonstration of a controller synthesized using one of the proposed methods would contribute positively to the paper.\\

\item \underline{Response to Comment \#3 of Reviewer 1:} We have revised the simulation section to consider a quadrotor with actuation constraints. We synthesized and verified a control barrier function-based control law using the approach of the manuscript, and showed how the input constraints affect the size of the safe region. Furthermore, we compared our synthesized CBF with a naive CBF that was not formally verified to demonstrate the effectiveness of our approach. In addition, we have added Section IV-G that describes how our proposed methods can be used to verify many state-of-the-art CBF synthesis techniques.\\

\item \underline{Comment \#4 of Reviewer 1:} When citing survey papers / textbooks please provide the specific result, e.g., [25, Theorem 4.3].\\

\item \underline{Response to Comment \#4 of Reviewer 1:} We have added chapter and/or result references to citations of books and survey papers.\\

\item \underline{Comment \#5 of Reviewer 1:} It would be nice to have both academic but also practical examples of when these methods could be used.\\

\item \underline{Response to Comment \#5 of Reviewer 1:} Positive invariance of safe regions must be verified in a variety of safety-critical applications, such as autonomous vehicle navigation and robotic manipulation. In both of these areas, it may be convenient to specify the express the safety region as a union of smaller subsets, each of which can be verified safe for a local approximation of the system dynamics. Our semi-algebraic framework is well-suited to this setting. This approach is taken by existing approaches that synthesize CBFs using dynamic programming and approximation of a value function. \\

\item \underline{Comment \#6 of Reviewer 1:} The literature review is somewhat weak. Please include information on why the cited papers relate to the results of this paper.\\

\item \underline{Response to Comment \#6 of Reviewer 1:} We have included additional references in the related work section of the revised manuscript and a more detailed summary of how the results relate to those in the present paper.  \\

\item \underline{Comment \#7 of Reviewer 1:} Please indicate which existing SOS-based heuristics are incomplete (paragraph 5).\\

\item \underline{Response to Comment \#7 of Reviewer 1:} We have revised pagagraph 5 to clarify the meaning of ``incomplete'', namely, the existing heuristics rely on a given nominal control policy.

\item \underline{Comment \#8 of Reviewer 1:} In Proposition 1: 
\begin{enumerate}
\item If it is guaranteed that an alpha exists based on the CBF definition 2, then this needs to be cited (converse CBF theorem?)
\item Need existence and uniqueness of solutions in order to use Nagumo’s Theorem.
\item Need an additional regularity condition based on the following counterexample:
- Consider a scalar double integrator system $\dot{x}_{1} = x_2$, $\dot{x}_{2} = u$ with a constraint function $b(x) = x_1^3$ and take the point $x_0 = [0 -1]$ where $b(x_0) = 0$ and $\dot{b}(x0) = 0 >= 0$.
\end{enumerate}

\item \underline{Response to Comment \#8 of Reviewer 1:} We thank the reviewer for identifying these points. With respect to the existence of $\alpha$ (denoted as $\kappa$ in the revised manuscript), we have added a separate result (Theorem 6) on existence of CBF-based safe control policies in our section on feedback controlled positive invariance. In the problem formulation, we have clarified that the goal is to ensure positive invariance whenever the solutions exist and are unique, rendering the Nagumo's Theorem results applicable. We further point out that, when the safe region is compact and the dynamics are polynomial (and hence locally Lipschitz), unique solutions are guaranteed to exist. Finally, we have added a regularity condition (Definition 7) which, in the case of a safe region defined by a single function $b$, reduces down to \emph{there does not exist $x$ satisfying $\frac{\partial b}{\partial x} = 0$ and $b(x) = 0$}.\\

\item \underline{Comment \#9 of Reviewer 1:} In Proposition 1:
\begin{enumerate}
    \item Needs more clarification.
\item Non-negativity of even polynomials is only NP-Hard if the degree is greater than or equal to 4
\end{enumerate}

\item \underline{Response to Comment \#9 of Reviewer 1:} Proposition 1 (now Proposition 8 in the revised manuscript) concerns the computational complexity of verifying viability of a given region. We prove that, for a simple definition of the system dynamics, the problem reduces to checking nonnegativity of a polynomial, which is known to be NP-hard. We thank the reviewer and add a statement to the theorem that the result is NP-hard when the degree of $f$ is greater than or equal to 4.\\

\item \underline{Comment \#10 of Reviewer 1:} In Definition 3, could you make it clearer what the $O(\cdot)$ term is?\\

\item \underline{Response to Comment \#10 of Reviewer 1:} We have removed this term from the revised manuscript and written the explicit formula for the higher-order Lie derivatives. \\

\item \underline{Comment \#11 of Reviewer 1:} In Theorem 1, should be intersection of indices from $0$ to $(r-1)$.\\

\item \underline{Response to Comment \#11 of Reviewer 1:} We thank the reviewer for identifying this error, which we have corrected.\\

\item \underline{Comment \#12 of Reviewer 1:} In Section III-C:

\begin{enumerate}
\item This should in general be clarified. Could benefit from additional notation, but also would be helpful to further elaborate on why the material in this section is relevant.
\item Sigma cone notation is somewhat confusing with summation notation.
\item We are under the impression that f and g in the system model need to be polynomial functions, and if this is indeed the case then it needs to be stated explicitly in the theorems. Further, please do not use f, g notation also to denote other polynomial functions.
\end{enumerate}

\item \underline{Response to Comment \#12 of Reviewer 1:} We thank the reviewer for these suggestions. We have clarified at the beginning of the section that the main contribution of the paper is proving that invariance of a semi-algebraic set can be represented as non-existence of solutions to systems of polynomial equations and inequalities, which we then map to convex SOS programs. The results of this section describe how non-existence of polynomial systems is equivalent to an SOS program. We have replaced the Sigma cone notation, and have stated in the system model of Section III that we consider polynomial systems. \\

\item \underline{Comment \#13 of Reviewer 1:} Theorem 4:
\begin{enumerate}
\item Would be helpful to have more information on where (5) comes from
\item In general, a non-negative polynomial need not be sum-of-squares. In light of this, the claims of both necessity and sufficiency need to be further clarified.
\item In summary, we do not understand this proof and feel that it needs to be further clarified.
\end{enumerate}

\item \underline{Response to Comment \#13 of Reviewer 1:} We have revised Theorem 4 to show that is a special case of a more general result that we prove in Section IV of the revised manuscript.  Eq. (5) of the original manuscript  follows by application of the Positivstellensatz to prove that there is no solution to the system (i) $b(x) = 0$, (ii) $\frac{\partial b}{\partial x}g(x) = 0$, and (iii) $\frac{\partial b}{\partial x}f(x) < 0$. \\

\item \underline{Comment \#14 of Reviewer 1:} In Section 4:
\begin{enumerate}
    \item  Sections 4B through 4F seem to just be concatenations of constraints that lead to more complicated SOS optimization problems. Could these sections be condensed into a more abstract result?
\item Should be clarified what exactly the admissible control set is.
\end{enumerate}

\item \underline{Response to Comment \#14 of Reviewer 1:} We thank the reviewer for this suggestion, which we have incorporated by reorganizing the manuscript. We first prove general results on verifying viability of a semialgebraic set in Section IV-A. We then derive SOS programs for the special cases of a single constraint set, intersection of simple sets, and unions of sets as corollaries of the more general result. In our work the admissible control set is of the form $\mathcal{U} = \{u \in \mathbb{R}^{m}: Au \leq c\}$ where $A \in \mathbb{R}^{p \times m}$ and $c \in \mathbb{R}^{p}$ are a known matrix and vector.\\

\item \underline{Comment \#15 of Reviewer 1:} Section 5: 
- Alternating descent approach: what variables are being minimized over? Do alpha, beta, eta require indices? Seems like they would not if they are decision variables. If they are not, please provide the update law.\\

\item \underline{Response to Comment \#15 of Reviewer 1:} We have written which variables are minimized over in the text immediately above each optimization problem formulation. We have not written the notations in the optimization problems themselves for ease of presentation.\\

\item \underline{Comment \#16 of Reviewer 1:} Simulation section:
\begin{enumerate}
\item Please expand. Actual evidence of simulation results would be helpful. Also, results for both verification and demonstration of synthesized controllers would improve the paper significantly.
\item Comparison with prior results, especially considering that it was stated in the introduction that the proposed methods improve upon the existing literature.
\end{enumerate}

\item \underline{Response to Comment \#16 of Reviewer 1:} We have significantly revised the simulation section to demonstrate our approach on CBF synthesis for a quadrotor with input constraints. We evaluate how tightening the constraints on the quadrotor control inputs changes the geometry of the safe region and also compare trajectories of a control law based on our synthesized CBF with a naive CBF.\\

\item \underline{Comment \#17 of Reviewer 1:} 
 Define what it means for b to be "a CBF for safety constraint C" in Problem 1.\\


\item \underline{Response to Comment \#17 of Reviewer 1:} We have revised Problem 1 to clarify that the goal is to verify viability of a given set $\mathcal{C}$.\\

\item \underline{Comment \#18 of Reviewer 1:} Are the last two conditions in Lemma 3 supposed to be for the same i?\\

\item \underline{Response to Comment \#18 of Reviewer 1:} Lemma 3 has been removed from the revised manuscript. We have clarified the notations and added examples to avoid confusion.\\

\item \underline{Comment \#19 of Reviewer 1:} What is uppercase L in (20)-(23)?\\

\item \underline{Response to Comment \#19 of Reviewer 1:} In this section of the manuscript, $L$ is the number of auxiliary state variables that are used to represent the trigonometric functions in the system dynamics.\\

\item \underline{Comment \#20 of Reviewer 1:} In the proof of Theorem 12, why is it sufficient for the sequence to be monotone nonincreasing? I think you need strictly monotone decreasing to apply the monotone convergence theorem? \\

\item \underline{Response to Comment \#20 of Reviewer 1:} In the case where the sequence is not strictly decreasing, there must be some $k$ where $\rho_{k} = \rho_{k}^{\prime}$, implying that $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$ and hence the algorithm terminates.\\

\item \underline{Comment \#21 of Reviewer 1:} Could Theorem 13 be extended to unions of CBFs?\\

\item \underline{Response to Comment \#21 of Reviewer 1:} We believe that the theorem could be extended to unions of CBFs. This is a promising direction of future work.\\

\item \underline{Comment \#22 of Reviewer 1:} In Theorem 14, can you explicitly define the "dual" operator *.\\

\item \underline{Response to Comment \#22 of Reviewer 1:} Theorem 14 has been removed from the revised manuscript.\\

\item \underline{Comment \#23 of Reviewer 1:} In the proof of Lemma 9, we think $\tilde{u}$ should be exponentially stabilizing, not simply stabilizing?\\

\item \underline{Response to Comment \#23 of Reviewer 1:} The reviewer is correct. We have updated the manuscript accordingly.\\

\end{itemize} 

==> First-revision/Response-document/Reviewer_7_comments.tex <==
\begin{center}
\textbf{Reviewer 7 Comments and Response}
\end{center}
~
\begin{itemize}
\item \underline{Initial Comments of Reviewer 7:} This is an interesting paper aimed at synthesizing and verifying CBFs
where safety regions are semi-algebraic. The author presents three
algorithms. The alternating descent approach, a fixed point approach,
and Newtonís method approach for synthesizing CBFs. The authors also
introduced trigonometric functions in their setting by converting these
into equality and inequality constraints. The setting involves a heavy
use sum-of-squares polynomials preservation, the positiveness of
polynomials on a semialgebraic set, Nagumo's theorem (as expected), and
duality via Farka's theorem. The work extends significatively the
author's work presented at the CDC conference in 2021. \\

\item \underline{Response to Initial Comments of Reviewer 7:} We thank the reviewer for taking the time to provide detailed comments. In what follows, we reproduce each comment, respond, and describe how the comment has been incorporated into the revised manuscript.\\

\item \underline{Comment \#1 of Reviewer 7:} The paper is quite dense and somewhat difficult to read despite the
fact that the reviewer has an idea of what is going on. CBFs are a
known topic and they can be motivated easily with practical examples.
Unfortunately, it seems that the author did not pay much attention to
motivating his results. I lost track of the number of polynomials that
had to be introduced, checked, and verified, to the point that I am not
sure if what the author has produced is tractable in an actual control
problem requiring CBFs. \\

\item \underline{Response to Comment \#1 of Reviewer 7:} We have revised the manuscript to motivate the results in the following manner. First, we discuss emerging applications of CBFs to applications in robotics, autonomous vehicles, and spacecraft navigation in the Introduction and Related Work section. Second, we discuss how our framework can be used to verify the safety properties of state-of-the-art CBF synthesis algorithms. Third, we present numerical examples within each section to illustrate the theoretical results, as well as a case study on CBF synthesis for quadrotor control.\\

\item \underline{Comment \#2 of Reviewer 7:} I think the results are relevant, but this can be my interest in CBFs
talking. The author should make this relevance clearer to a broader
audience with a good motivation of the need for the semialgebraic
setting he has introduced. Hence, the paper needs a major revision. To
begin with, I would move most proof and intermediate results to an
appendix. This way the flow of results will be clearer for the reader
and will allow for motivating examples in all sections of the paper.
This is the case in most of the papers cited by the author on CBFs. Overall, the paper has a lot of potential for publication in TAC, but
not in the current format. Motivation, examples, re-formatting, and a
relevant control application are needed. I look forward to seeing the
next iteration of this work.\\

\item \underline{Response to Comment \#2 of Reviewer 7:} As discussed in the previous response, we have clarified how semialgebraic sets are broadly applicable and encompass many of the standard CBF constructions, including high-order CBFs, neural CBFs, and constructing CBFs from approximations of the reach-avoid value function. We thank the reviewer for providing advice on improving the presentation and readability of the paper. We have moved the proofs to Appendices and added illustrative numerical examples throughout the text.\\



\item \underline{Comment \#3 of Reviewer 7:} Unclear when f and g are continuous functions (like in (1) ) and when
f's and g's are polynomials. This could be just a notation issue. But
it can be clarified later when Lie derivatives of g and b are taken to
show positive invariance. For instance, in Proposition 2's proof, f and
g are defined by components but the reader does not know if these
should be polynomials as declared in the previous section.\\  

\item \underline{Response to Comment \#3 of Reviewer 7:} We have revised the system model in Section III-A to clarify that $f$ and $g$ are polynomials. The only exception is in Section IV-F, where we consider systems with trigonometric functions in the dynamics.\\

\item \underline{Comment \#5 of Reviewer 7:} "If and only if" vs "iff" (e.g., Proposition 1 vs Theorem 4).\\

\item \underline{Response to Comment \#5 of Reviewer 7:} We have revised the manuscript to consistently use ``if and only if'' for clarity.\\

\item \underline{Comment \#6 of Reviewer 7:} Theorem vs propositions Theorem 4 vs proposition 4. What makes
something a Theorem and what makes something a proposition? \\

\item \underline{Response to Comment \#6 of Reviewer 7:} In general, we use theorems to denote more significant main results or results that have more complicated proofs. \\

\item \underline{Comment \#7 of Reviewer 7:} Conditions that require testing the nonexistence of a function are
difficult to use (e.g., Lemma 4 and others). \\

\item \underline{Response to Comment \#7 of Reviewer 7:} The reviewer is correct that testing nonexistence is challenging. We emphasize that our results enable safety verification by showing \emph{existence} of polynomials satisfying a set of sum-of-squares constraints, thus providing a safety certificate for a system. Indeed, a key contribution of our work is using theorems of alternatives to transform non-existence conditions (which are difficult to verify) to existence conditions that can be formulated as optimization problems. On the other hand, since solving SOS programs in practice requires limiting the degree of the polynomials, it may not be possible to conclude that a system is \emph{unsafe} simply because a feasible certificate could not be found.\\

\item \underline{Comment \#8 of Reviewer 7:} Theorem 8 has conditions that seem difficult to test. Existence of
polynomials?\\

\item \underline{Response to Comment \#8 of Reviewer 7:} The existence of the polynomials satisfying the conditions of the theorems can be verified by solving sum-of-squares programs, which can be mapped to semidefinite programs and solved using open-source toolboxes such as SOStools for Matlab. As noted in the previous response, however, whether the solver is able to find polynomials satisfying the conditions may depend on the choice of monomial basis, for example, if the degrees of the polynomials in the search space are sufficiently large. This is a limitation of our approach that we acknowledge in the paper.\\

\item \underline{Comment \#9 of Reviewer 7:} 2nd equation first paragraph page 7, nonstandard notation for a
definition of $z'_{ij}$.	\\

\item \underline{Response to Comment \#9 of Reviewer 7:} We have removed this notation.\\

\item \underline{Comment \#10 of Reviewer 7:} Paper about keeping positive invariance. Most proofs by
contradiction. These seem like non-testable conditions. Can these be
actually tested for particular systems with semialgebraic safety
constraints? Is the tractability of the author's results follow from
the HOCBF?  So, only the $\psi$ functions need to be checked/verified? \\

\item \underline{Response to Comment \#10 of Reviewer 7:} We emphasize that, if a set of polynomials can be found that satisfy the SOS feasibility conditions described in the paper, then the semi-algebraic set is verified to be positive invariant. Furthermore, if the set is invariant and the degree of the polynomials is sufficiently large, then a solution to the feasibility conditions is guaranteed to exist.\\

Verifying semi-algebraic sets with large numbers of polynomials and/or high-degree polynomials may be intractable, and indeed includes several known hard problems as special cases. We describe some special cases in Section IV-C, such as HOCBFs pointed out by the reviewer, that may be tractable to verify.\\

\item \underline{Comment \#11 of Reviewer 7:} Codifies trigonometric functions as polynomials. And thus, these can
be introduced into the semi-algebraic framework as inequality and
equality constraints on states and inputs.\\

\item \underline{Response to Comment \#11 of Reviewer 7:} We thank the reviewer for the comment.\\

\item \underline{Comment \#12 of Reviewer 7:} Despite the fact that CBFs are well known already in the community.
This paper, due to its length, lack motivating examples right after
each of the multiple results presented. \\

\item \underline{Response to Comment \#12 of Reviewer 7:} We have added numerical examples after the results as well as a set of motivating examples (Section IV-A) of how existing CBF constructions can be verified as special cases of our methods. We have also added a numerical case study on safe control of a quadrotor UAV.\\

\item \underline{Comment \#13 of Reviewer 7:} Proof of Proposition 5, $\mu$ is the control policy. But then u is
used. Is this a typo? is $\mu$ a polynomial as described earlier with the
$\mu$ notation? Perhaps an overall review of the notation is required
including a section establishing notation right after the introduction.
Proof of Lemma 3, uses $\mu$.\\

\item \underline{Response to Comment \#13 of Reviewer 7:} We have removed this notation from the paper.\\

\item \underline{Comment \#14 of Reviewer 7:} Lemma 4 proof should be provided.\\

\item \underline{Response to Comment \#14 of Reviewer 7:} We have reorganized the paper significantly. Lemma 4 no longer appears.\\

\item \underline{Comment \#15 of Reviewer 7:} It is really difficult to assess the practicality of Theorem 8
without further discussion of its practicality in an illustrative
example.\\

\item \underline{Response to Comment \#15 of Reviewer 7:} As discussed above, we have discussed practicality of the approach in the paper and added more examples.\\

\item \underline{Comment \#16 of Reviewer 7:} In Lemma 7, is the minimization of $u^Tz$ constrained or unconstrained?
If constrained, are these convex, polynomial? will these be (32) and
(33)? This has to be satisfied for all x, right? or is the Lie
derivative evaluated at a point? \\

\item \underline{Response to Comment \#16 of Reviewer 7:} Lemma 7 has been removed from the revised manuscript.\\


\item \underline{Comment \#17 of Reviewer 7:} In Lemma 9, in what sense $(x^{\ast}, u^{\ast})$ is a fixed point? is
it an equilibrium? \\

\item \underline{Response to Comment \#17 of Reviewer 7:} The reviewer is correct, it is an equilibrium point. We have changed the terminology to ``equilibrium'' throughout the paper.\\


\item \underline{Comment \#18 of Reviewer 7:} Subindex X is missing in the Frechet derivative eq (48). What is (49)? a matrix function? Is $F_2$ a row with $F_{22}$ part of it?
The notation is confusing here. It appears the author was running out
of steam by this point.\\

\item \underline{Response to Comment \#18 of Reviewer 7:} We have removed the Newton's method from the paper, as it was found to give trivial results in simulations that we attempted.\\


\item \underline{Comment \#19 of Reviewer 7:} Overall, many commas and periods are missing.\\

\item \underline{Response to Comment \#19 of Reviewer 7:} We have carefully proofread and revised the paper to improve grammar and syntax.\\


\item \underline{Comment \#20 of Reviewer 7:} This paper will make more sense if all proofs are given in an
appendix.\\

\item \underline{Response to Comment \#20 of Reviewer 7:} We have moved the proofs to appendices as suggested by the reviewer.\\


\item \underline{Comment \#21 of Reviewer 7:} Section VI is an afterthought. The author provided 3 synthesis
methods. None of them seemed to have been exercised. What theorem,
proposition, or algorithm was used in Section VI? How was the SOS
toolbox used? Did [34] have the author's work implemented?  Please
clarify.\\

\item \underline{Response to Comment \#21 of Reviewer 7:} We carried out a new case study on control of a quadrotor UAV, in which we analyzed how tightening constraints on the control inputs affected the size of the safe region. SOStools was used to solve the sum-of-squares optimization problems to construct and verify the invariant set $\mathcal{C}$.\\


\end{itemize}

==> First-revision/Response-document/Reviewer_8_comments.tex <==
\begin{center}
\textbf{Reviewer 8 Comments and Response}
\end{center}
~
\begin{itemize}
\item \underline{Initial Comments of Reviewer 8:} This manuscript proposes an interesting approach for a semi-algebraic
framework for verification and synthesis of control barrier functions.
Overall, the paper is well written, and contain potentially useful
results. Some suggestions to improve the quality of the paper are as
follows. \\

\item \underline{Response to Initial Comments of Reviewer 8:} We thank the reviewer for taking the time to provide detailed comments. In what follows, we reproduce each comment, respond, and describe how the comment has been incorporated into the revised manuscript.\\

\item \underline{Comment \#1 of Reviewer 8:} In the paper, some terminologies should be defined formally. For
instance, we need to define the "positive invariance" and class-K
function in page 2.\\

\item \underline{Response to Comment \#1 of Reviewer 8:} We have provided definitions for both terms in Section III-A of the revised manuscript.\\

\item \underline{Comment \#2 of Reviewer 8:} When introducing the CBF in equation (2), it would be more helpful
to explain some intuitive meaning of the equation (2) and the CBF. Is
it similar to Lyapunov function?\\

\item \underline{Response to Comment \#2 of Reviewer 8:} Intuitively, a CBF constraints the control input to ensure that the Lie derivative of the function $h(x)$ is nonnegative on the boundary of $\{x: h(x) \geq 0\}$, in order to ensure that this set is positive invariant. It is similar to a Lyapunov function, and indeed both methods are often grouped together in the framework of energy-based methods. We have added more intuitive description after the definition of CBF.\\


\item \underline{Comment \#3 of Reviewer 8:} In equation (25), it would be better if the Euler-Lagramge dynamics
is briefly introduced for readers who do not know about it. \\

\item \underline{Response to Comment \#3 of Reviewer 8:} We thank the reviewer for the comment. After careful consideration, we decided to remove the Euler-Lagrange dynamics from the manuscript in order to make room for additional descriptions and examples of the main results.\\


\item \underline{Comment \#4 of Reviewer 8:} It would be better to clearly indicate that the convergence in
Theorem 12 is local convergence. \\

\item \underline{Response to Comment \#4 of Reviewer 8:} We have removed the Newton's method algorithm from the paper, as it performed poorly in simulations that we conducted.\\


\item \underline{Comment \#5 of Reviewer 8:} Before Lemma 9, it would be better to introduce the definition of
the fixed point. It is not clearly explained in the paper. \\

\item \underline{Response to Comment \#5 of Reviewer 8:} We refer to a fixed point as any point $x^{\ast}$ such that there exists $u^{\ast}$ with $f(x^{\ast}) + g(x^{\ast})u^{\ast} = 0$. We have added this explanation to the revised manuscript.\\


\item \underline{Comment \#6 of Reviewer 8:} In Lemma 9, it is not clear what would be the definition of the
controllability for the general nonlinear system in (1).\\

\item \underline{Response to Comment \#6 of Reviewer 8:} In this result, we require only controllability of the linearized model around the equilibrium point. We have clarified this in the paper.\\


\item \underline{Comment \#7 of Reviewer 8:} Under equation (47), it is stated the equation (46) and (47) are
special cases. It would be better to discuss how these approximations
can introduce conservativeness. \\

\item \underline{Response to Comment \#7 of Reviewer 8:} As discussed above, we have removed the Newton's method algorithm from the paper, as it performed poorly in simulations.\\

 
 \item \underline{Comment \#8 of Reviewer 8:} Overall, it would be better if the readability of the paper is
improved for the readers who are not familiar with the materials.\\

\item \underline{Response to Comment \#8 of Reviewer 8:} We have improved the readability of the manuscript by moving proofs to appendices, adding examples, and providing a more detailed case study as well as improving the overall presentation. We thank the reviewer for the comments that helped us to improve the paper contents.

\end{itemize}

==> Introduction.tex <==
\section{Introduction}
\label{sec:intro}
Safety is a critical property of autonomous control systems in medical, manufacturing, transportation, and other vital applications. From a control-theoretic perspective, safety is typically characterized by positive invariance of a particular safe region, for example, ensuring that a vehicle remains a desired safe distance from humans or obstacles, or maintaining the temperature of a system within tolerated limits. Methodologies such as energy-based methods \cite{dawson2022safe}, counterexample-guided synthesis \cite{henzinger2003counterexample}, and abstraction-based verification \cite{ratschan2007safety} have been proposed to verify system safety and design safe control algorithms.

Among these techniques, energy methods such as control barrier functions and barrier certificates have attracted significant research attention \cite{prajna2007framework,ames2019control,krstic2021inverse}. These methods map the safety constraint to a barrier function such that the system is safe if the barrier function is nonnegative. The control input is then chosen to ensure that the derivative of the barrier function is nonnegative at the boundary of the safe region. The main advantage of this approach is that it provides safety guarantees while also being minimally invasive, since additional control effort is only needed as the system approaches the safety boundary.

While CBFs have shown great promise in a variety of applications including bipedal locomotion \cite{hsu2015control}, autonomous driving \cite{he2022autonomous}, and spacecraft rendezvous \cite{agrawal2021safe}, challenges remain. One practical difficulty is that there may not be a control input to satisfy the barrier function constraint at each time instant, which may lead to safety violations. This is the challenge of \emph{verifying} a CBF. While some sufficient heuristic methods based on convex sum-of-squares optimization have been proposed \cite{santoyo2019verification,jagtap2020compositional}, they are not complete, i.e., they may fail to verify a CBF even if the CBF is valid. These challenges are especially salient for systems with actuation constraints and non-polynomial dynamics.

Another related challenge is synthesizing CBFs that will ensure a desired safety constraint.  Typically, CBFs are constructed using trial-and-error or domain knowledge. While approaches to synthesizing CBFs using alternating descent sum-of-squares \cite{ames2019control} and neural networks \cite{wang2021learning,peruffo2021automated} are promising, these algorithms are not guaranteed to return a CBF with verifiable safety guarantees.

In this paper, we propose a semialgebraic optimization framework for verification and synthesis of CBFs. In our verification framework, we consider two types of safety properties. First, we consider viability, defined as the existence of a (possibly discontinuous) control policy that ensures positive invariance of a given set. We use the Positivstellensatz from real algebraic geometry to derive exact sum-of-squares conditions for viability, and derive viability conditions for single CBFs, intersections of CBFs, high-order CBFs, and unions of CBFs as special cases. We show that several state-of-the-art synthesis algorithms result in CBFs that can be verified by our framework.  We then consider the problem of verifying existence of a continuous feedback control policy that ensures safety. We develop sufficient sum-of-squares conditions and construct a safe feedback control policy by exploiting semi-algebraic triangulations.

%On the verification side, we first show that the verification problem is NP-hard and that existing SOS-based heuristics are incomplete. We then formulate exact SOS conditions for a function to be a CBF  using the Positivstellensatz, which is a result from algebraic geometry that gives equivalent conditions for existence of solutions to systems of polynomial equations and inequalities. We generalize our approach to derive exact (albeit high-dimensional) SOS programs for intersections of multiple CBFs, high-order CBFs, semi-algebraic sets, actuation-constrained systems, and systems with Euler-Lagrange dynamics. We also propose a sufficient approach for systems with trigonometric dynamics. These generalizations ensure that our framework is applicable to a variety of different constraints, safe regions, and system dynamics that may arise in practical applications of safe control.

On the synthesis side, we propose three algorithms. The first is an alternating descent approach, similar to \cite{jagtap2020compositional}, which we generalize to high-order CBFs. The second constructs local CBFs for systems with fixed points, with driftless systems as an important special case. 

The paper is organized as follows. Section \ref{sec:related} presents the related work. Section \ref{sec:model} presents the system model and background material. Section \ref{sec:verification} presents a convex, semi-algebraic framework for verification of CBFs. Section \ref{sec:synthesis} presents algorithms for synthesizing CBFs. Section \ref{sec:simulation} presents simulation results. Section \ref{sec:conclusion} concludes the paper.

==> Model.tex <==
\section{Model and Preliminaries}
\label{sec:model}
This section presents the system model and needed background.

\subsection{System Model}
\label{subsec:model}
We consider a nonlinear control system with dynamics 
\begin{equation}
\label{eq:dynamics}
\dot{x}(t) = f(x(t)) + g(x(t))u(t)
\end{equation}
where $x(t) \in \mathbb{R}^{n}$ denotes the state, $u(t) \in \mathbb{R}^{m}$ is a control input, and $f: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n}$ and $g: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n \times m}$ are continuous functions. Throughout the paper, we let $[x]_{i}$ denote the $i$-th element of $x \in \mathbb{R}^{n}$.

The system is required to remain in a safe region $\mathcal{C}$, which is defined by $\mathcal{C} = \bigcap_{i=1}^{M}{\{x : h_{i}(x) \geq 0\}}$ for some functions $h_{1},\ldots,h_{M}: \mathbb{R}^{n} \rightarrow \mathbb{R}$. %We say that a control policy $\mu: \mathbb{R}^{n} \rightarrow \mathbb{R}^{m}$ ensures safety if there exists a set $\tilde{\mathcal{C}} \subseteq \mathcal{C}$ such that 
We define a safe control policy as follows.
\begin{definition}
\label{def:safe-control-policy}
A function $\mu: \mathbb{R}^{n} \rightarrow \mathbb{R}^{m}$ is a safe control policy if (i) there exists a set $\tilde{\mathcal{C}}$ with $\tilde{\mathcal{C}} \subseteq \mathcal{C}$, and (ii) for any $x(0) \in \tilde{\mathcal{C}}$, if $u(t) = \mu(x(t))$ for all $t \geq 0$, then $\tilde{\mathcal{C}}$ is positive invariant.
\end{definition}

A set is controlled positive invariant (CPI) if it is positive invariant for some control policy $\mu$.


\subsection{Background on Control Barrier Functions}
\label{subsec:CBF-background}
Control Barrier Functions (CBFs) have been proposed to ensure safety of nonlinear systems, and are defined as follows.

\begin{definition}
\label{def:CBF}
A function $b$ is a control barrier function for (\ref{eq:dynamics}) if there is a class-K function $\alpha$ such that, for all $x$ with $b(x) \geq 0$, there exists $u$ satisfying 
\begin{equation}
\label{eq:CBF-def}
\frac{\partial b}{\partial x}(f(x) + g(x)u) \geq -\alpha(b(x)).
\end{equation}
\end{definition}
The following result gives a safety proof for systems with CBFs.
\begin{theorem}[\cite{ames2019control}] 
\label{theorem:CBF-safety}
Suppose that $b$ is a CBF, $b(x(0)) \geq 0$, and $u(t)$ satisfies (\ref{eq:CBF-def}) for all $t$. Then the set $\{x : b(x) \geq 0\}$ is positive invariant.
\end{theorem}
As a consequence of Theorem \ref{theorem:CBF-safety}, if $b(x)$ is a CBF with $\{b(x) \geq 0\} \subseteq \{h_{i}(x) \geq 0\}$ for $i=1,\ldots,M$, then any control policy that satisfies (\ref{eq:CBF-def}) is a safe control policy. One challenge with CBF-based control policies is that the constraint (\ref{eq:CBF-def}) may become infeasible if $\frac{\partial b}{\partial x}g(x) = 0$. High-order CBFs (HOCBFs), defined as follows, have been proposed to address this limitation.
\begin{definition}[\cite{xiao2021high}]
\label{def:HOCBF}
For a function $b$, define functions $\psi_{0},\ldots,\psi_{r}$ by 
\begin{IEEEeqnarray*}{rCl}
\psi_{0}(x) &=& b(x) \\
\psi_{1}(x) &=& \dot{\psi}_{0}(x) + \alpha_{1}(\psi_{0}(x)) \\
 &\vdots& \\
 \psi_{r}(x) &=& \dot{\psi}_{r-1}(x) + \alpha_{r}(\psi_{r-1}(x))
 \end{IEEEeqnarray*}
 where $\alpha_{1},\ldots,\alpha_{r}$ are class-K functions. Define $\mathcal{C}_{i}$ by $\mathcal{C}_{i} = \{x : \psi_{i}(x) \geq 0\}$ for $i=0,\ldots,r$. The functions $b,\psi_{1},\ldots,\psi_{r}$ define a HOCBF if $\frac{\partial \psi_{i}}{\partial x}g(x) = 0$ for $i < r$ and, for all $x \in \bigcap_{i=0}^{r}{\mathcal{C}_{i}}$, there exists $u$ satisfying
 \begin{equation}
 \label{eq:HOCBF-def}
 L_{f}^{r}b(x) + L_{g}L_{f}^{r-1}b(x)u + O(b(x)) + \alpha_{m}(\psi_{r-1}(x)) \geq 0
 \end{equation}
 where $O(b(x))$ denotes lower-order Lie derivatives of $b(x)$.
 \end{definition}
 The following result establishes safety of HOCBFs.
 \begin{theorem}[\cite{xiao2021high}]
 \label{theorem:HOCBF-safety}
 If $b$ is a HOCBF, then the set $\bigcap_{i=0}^{r}{\mathcal{C}_{i}}$ is positive invariant under any control policy that satisfies (\ref{eq:HOCBF-def}) for all $x \in \bigcap_{i=0}^{r}{\mathcal{C}_{i}}$.
 \end{theorem}
 As a corollary to Theorem \ref{theorem:HOCBF-safety}, if $\bigcap_{i=0}^{r}{\mathcal{C}_{i}} \subseteq \mathcal{C}$ and $b(x)$ is an HOCBF, then any control policy satisfying (\ref{eq:HOCBF-def}) is a safe control policy.
 
 \subsection{Preliminary Results}
 \label{subsec:preliminary}
 We now give two needed background results, namely, the Positivstellensatz and Farkas's Lemma. Recall that a Sum-of-Squares (SOS) polynomial is a polynomial $f(x)$ such that $$f(x) = \sum_{i=1}^{k}{g_{i}(x)^{2}}$$ for some polynomials $g_{1}(x),\ldots,g_{k}(x)$. Selecting coefficients of $f(x)$ to ensure that $f(x)$ is SOS can be represented as a semidefinite program, a procedure known as SOS optimization \cite{parrilo2003semidefinite,ahmadi2017improving}. The cone  $\Sigma[q_{1},\ldots,q_{k}]$ associated with polynomials $q_{1},\ldots,q_{k}$ is equal to the set of polynomials $f$ with $$f(x) = p_{0}(x) + \sum_{i=1}^{N}{p_{i}(x)\beta_{i}(x)},$$ where $p_{0},\ldots,p_{N}$ are SOS and $\beta_{1},\ldots,\beta_{N}$ are products of powers of the $q_{i}$'s. For a set of polynomials $f_{1},\ldots,f_{N}$, we define the ideal generated by the polynomials as $$\mathcal{I}[f_{1},\ldots,f_{N}] = \left\{\sum_{i=1}^{N}{\eta_{i}f_{i}} : \eta_{1},\ldots,\eta_{N}\right\}.$$
 
 The Positivstellensatz, stated as follows, gives equivalent conditions for existence of solutions to systems of polynomial equations and inequalities.
 \begin{theorem}[Positivstellensatz \cite{bochnak2013real}]
 \label{theorem:Psatz}
 Consider a collection of polynomials $\{f_{j}: j=1,\ldots,r\}$, $\{g_{i} : i=1,\ldots,m\}$ and $\{h_{k} : k=1,\ldots,s\}$. Then the set 
 \begin{multline*}
 \left(\bigcap_{j=1}^{r}{\{x : f_{j}(x) \geq 0\}}\right) \cap \left(\bigcap_{i=1}^{m}{\{x : g_{i}(x) = 0\}}\right) \\
 \cap \left(\bigcap_{k=1}^{s}{\{x : h_{k}(x) \neq 0\}}\right)
 \end{multline*}
 is empty if and only if there exist polynomials $f$, $g$, and $h$ satisfying (i) $f(x) \in \Sigma[f_{1},\ldots,f_{r}]$, (ii) $g(x) \in \mathcal{I}[g_{1},\ldots,g_{m}]$,  (iii) $h$ is a product of powers of the $h_{k}$'s, and (iv) $f(x) + g(x) + h(x)^{2} = 0$ for all $x$.
 \end{theorem}

When the $f_{j}$'s, $g_{i}$'s, and $h_{k}$'s are given, attempting to find solutions of the equation $f(x) + g(x) + h(x)^{2} = 0$ is an SOS optimization problem \cite{parrilo2003semidefinite}.
 
 Finally, Farkas's Lemma is as follows.
 \begin{lemma}[Farkas's Lemma \cite{dinh2014farkas}]
 \label{lemma:Farkas}
 Let $A \in \mathbb{R}^{m \times n}$ and $b \in \mathbb{R}^{m}$. Then exactly one of the following is true:
 \begin{enumerate}
 \item There exists $x \in \mathbb{R}^{n}$ with $Ax \leq b$
 \item There exists $y \in \mathbb{R}^{m}$ with $A^{T}y = 0$, $b^{T}y < 0$, and $y \geq 0$.
 \end{enumerate}
 \end{lemma}
Farkas's Lemma gives equivalent conditions for existence of solutions of linear inequalities. 


==> Response-document/Reviewer_5_comments.tex <==
\begin{center}
\textbf{Reviewer 5 Comments and Response}
\end{center}
~
\begin{itemize}

\item \underline{Initial Comments of Reviewer 5:} The author has reorganized the presentation more friendly for the
reader, which has clarified the presentation and readability. Also,
examples and a new simulation study have been presented. However, the
mechanics of how to apply the methods described need more work. Also,
the methods are applied to a linearized model (why not a simple
differential drive?) and use a barrier function that does not
illustrate the author's result. For example, the author provides an
algorithm for CBF (and HOCBF) synthetization that has not been
demonstrated nor shown that these produce less complexity than solving
the SOS problem directly. 

This reviewer still thinks the work could be suitable for publication
in TAC, but more work is required in the latter sections of the
manuscript.\\

\item \underline{Response to Initial Comments of Reviewer 5:} We thank the reviewer for taking the time to give detailed comments, which have greatly improved the quality of the manuscript. Our responses are given as follows.\\

\item \underline{Comment \#1 of Reviewer 5:} Paragraph after (1), should b be c?\\


\item \underline{Response to Comment \#1 of Reviewer 5:} The reviewer is correct. We thank the reviewer for identifying this typo.\\

\item \underline{Comment \#2 of Reviewer 5:} Should there be coefficients in the equation for f(x) after (4)? The
author mentions selecting coefficients of f(x) in the paragraph
following the f(x) definition. Or is he talking about the $g_i$'s
polynomials?\\

\item \underline{Response to Comment \#2 of Reviewer 5:} The term ``coefficients'' refers to the coefficients of the polynomial $f(x)$, not coefficients of the $g_{i}$'s in the un-numbered equation referenced by the reviewer. Hence coefficients are not needed in this equation. We have created a new paragraph starting with ``Selecting coefficients of f(x)...'' to minimize confusion.\\

\item \underline{Comment \#3 of Reviewer 5:} I might have missed it, but why is $\psi$ a scalar (function?) in the
proof of Proposition 2?\\

\item \underline{Response to Comment \#3 of Reviewer 5:} The gradient $\frac{\partial b}{\partial x}$ is a $1 \times n$ row vector, while $f(x) \in \mathbb{R}^{n}$. Hence $\psi = \frac{\partial b}{\partial x}f(x)$ has dimension $1 \times 1$ and is a scalar.\\

\item \underline{Comment \#4 of Reviewer 5:} Add numbers to examples. \\

\item \underline{Response to Comment \#4 of Reviewer 5:} We thank the reviewer for the formatting suggestion. We have added numbers to the examples in the revised manuscript.\\

\item \underline{Comment \#5 of Reviewer 5:} Example after Proposition 4, the author mentions 2 sets but then gives
4 sets. Did you mean pairs or something else? Then in the note that
follows   $\{2,4\}$ gives non-viability of C. Please clarify.\\

\item \underline{Response to Comment \#5 of Reviewer 5:} The reviewer is correct, this is a typo. It should be ``four sets'' instead of ``two sets''. We have revised the manuscript to correct this error.\\

\item \underline{Comment \#6 of Reviewer 5:} Should Proposition 7 be a corollary?\\

\item \underline{Response to Comment \#6 of Reviewer 5:} We have restated Proposition 7 as a corollary, and also added a brief proof to show how the corollary follows from the theorem.\\

\item \underline{Comment \#7 of Reviewer 5:} The statement in the proof of proposition 9 "NP-hardness of Problem 1
is weaker than NP-hardness of checking whether there exists x satisfying
the conditions of Proposition 2" should be clarified.  \\

\item \underline{Response to Comment \#7 of Reviewer 5:} For clarity, the statement has been  revised to, ``If there is a polynomial-time algorithm for Problem 1, then that algorithm can be used to check the conditions of Proposition 2, since viability of a set $\{x: b(x) \geq 0\}$ for some polynomial $b(x)$ is a special case of viability of a practical algebraic set $\mathcal{C}$. Hence, in order to prove that Problem 1 is NP-hard, it suffices to prove that checking the conditions of Proposition 2 is NP-hard.''\\



\item \underline{Comment \#8 of Reviewer 5:} The use of Theorem and/or Proposition for the author's result is
inconsistent (e.g., Theorem 5 and Proposition 9) Why is one a Theorem
and the other a proposition?\\

\item \underline{Response to Comment \#8 of Reviewer 5:} We have revised the paper to use the term ``Theorem'' for main results and ``Lemma'' for results that are used to prove theorems.\\

\item \underline{Comment \#9 of Reviewer 5:} Are there no conditions whatsoever on J in Theorem 6?\\

\item \underline{Response to Comment \#9 of Reviewer 5:} The reviewer is correct. The only condition on $J$ is the existence of a solution to the optimization problem, which is required for the optimization-based control policy to be well-defined.\\

\item \underline{Comment \#10 of Reviewer 5:} Last line in Th. 6 proof, .... (11)-(14) "hold" everywhere (?)\\

\item \underline{Response to Comment \#10 of Reviewer 5:} The reviewer is correct. We thank the reviewer for identifying this omission.\\

\item \underline{Comment \#11 of Reviewer 5:} Theorem 7 statement, explicitly specify the phrase "the assumptions of
this subsection". Also, what is $\hat{C}$? Positive invariant set for the
augmented system?\\

\item \underline{Response to Comment \#11 of Reviewer 5:} For brevity of the theorem statement, we have added a numbered Assumption to the beginning of Section IV-F, and referenced that assumption in the statement of Theorem 7.\\

\item \underline{Comment \#12 of Reviewer 5:} Section IV seems out of place in that it does a literature review of
CBF applications. Move to the problem statement or some appropriate
preliminary section.\\

\item \underline{Response to Comment \#12 of Reviewer 5:} The goal of this section is to show that several safety filter constructions in the existing literature can be verified as special cases of our framework. We have moved this discussion to Section IV-G.\\

\item \underline{Comment \#13 of Reviewer 5:} It is not clear how $\rho'$ enters (18) and (19). Is it the result of
the optimization at a previous time? It would be clearer if the author
described the approach using pseudocode. In the proof of Th. 8, it is
mentioned that $\rho'$ and $\rho$ are solutions of (18) and (19),
respectively. So, some clarification should be provided on how to run
the algorithm. It is also unclear to this reviewer how $\rho_k$ is
monotonically nonincreasing and always negative. Is it due to the
choice of the SOS $\Lambda$? if so, how is it chosen? The same question
is posed for the HOCBF synthesis.\\

\item \underline{Response to Comment \#13 of Reviewer 5:} The reviewer is correct. $\rho^{\prime}$ is the solution to the previous optimization problem. We will provide a pseudocode description of the algorithm.\\

We have that $\rho$ and $\rho^{\prime}$ are monotonically increasing because, at step $k$, $\rho_{k-1}$, $\alpha^{k-1}$, $\eta^{k-1}$, $\theta_{1}^{k-1},\ldots,\theta_{m}^{k-1}$, $w^{k-1}$, and $\beta^{k-1}$ comprise a feasible solution to (18). Similarly, $b^{k-1}$ and $\rho_{k-1}$ are feasible solutions to (19). Hence, at each iteration, the value of the optimization problem is bounded below by the value of the previous iteration.

In general, we are not guaranteed that $\rho_k$ is negative. Rather, as stated in Thoerem 8, if $\rho_{k}$ is negative, then $b$ is a valid CBF.\\

\item \underline{Comment \#14 of Reviewer 5:} Section VI, the author exercised his approach for a simple algebraic
b(x) for a linearized quadcopter system. Unfortunately, this example
does not fully illustrate the extent of the author's presented results.
That is, the system is expected to exhibit nonlinearities (e.g.,
trigonometric) and that more complex CBFs or HOCBFs be exercised. Also,
a comparison of the complexity between the proposed algorithms and that
of the direct SOS problem should be provided.  \\

\item \underline{Response to Comment \#14 of Reviewer 5:} We thank the reviewer for the comment. We have revised the simulation section to include two new case studies. The first case study shows the viability verification of a semi-algebraic set for a six-dimensional nonlinear system (2-D quadrotor) with trigonometric dynamics. The second case study demonstrates our alternating-descent synthesis algorithm on a three-dimensional nonlinear system, namely a power converter. The case study evaluates the convergence of the alternating descent approach for different (infeasible) initializations of the CBF. Further details of the evaluation are contained in Section VI of the revised manuscript.

\end{itemize}

==> Synthesis-v2.tex <==
\section{Problem Formulation: CBF Synthesis}
\label{sec:synthesis}
This section considers the following problem.
\begin{problem}
\label{problem:synthesis}
Given a safety constraint $\mathcal{C} = \{x: h(x) \geq 0\}$, construct a CBF $b: \mathbb{R}^{n} \rightarrow \mathbb{R}$ or family of CBFs $b_{1},\ldots,b_{M}$ that guarantee safety with respect to $\mathcal{C}$.
\end{problem}

We present three approaches to synthesizing CBFs. The first approach uses an alternating descent method. The second approach exploits the existence of fixed points to construct CBFs for local neighborhoods. The third approach uses Newton's method in function space to guarantee local convergence to a CBF.

\subsection{Alternating Descent Approach}
\label{subsec:ad-synthesis}
Our first approach is based on the SOS constraints introduced in Section \ref{sec:verification}. When the function $b(x)$ is unknown, the constraints become  non-convex. We therefore propose an alternating-descent heuristic, in which we alternate between updating the CBF candidate $b(x)$ and the polynomials used for verification. We describe our approach for synthesizing CBFs for polynomial dynamics, although a similar approach can be exploited for systems with Lagrangian dynamics or dynamics with trigonometric functions.

We initialize a function $b^{0}(x)$ arbitrarily (e.g., $b^{0}(x) = h_{i}(x)$ for some $i$) and initialize parameters $\rho_{0}$ and $\rho_{0}^{\prime}$ to be infinite. At step $k$, we solve the following SOS program with variables $\rho$, $\alpha^{k}(x)$, $\eta^{k}(x)$, $\theta_{1}^{k}(x),\ldots,\theta_{m}^{k}(x)$, $w(x)$, and $\beta^{k}(x)$:

\begin{equation}
\label{eq:alternating-descent-1}
\begin{array}{ll}
\mbox{minimize} & \rho \\
\mbox{s.t.} & \alpha^{k}(x)\frac{\partial b^{k-1}}{\partial x}f(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)\left[\frac{\partial b^{k-1}}{\partial x}g(x)\right]_{i}} \\
& + \eta^{k}(x)b^{k-1}(x) + \rho \Lambda(x) - 1 \in SOS \\
& -\beta^{k}(x)b^{k-1}(x) + w(x)h(x) - 1 \in SOS \\
& \beta^{k}(x), \alpha^{k}(x) \in SOS
\end{array}
\end{equation}

In (\ref{eq:alternating-descent-1}), $\Lambda(x)$ is an SOS polynomial chosen to ensure that the first constraint is SOS for sufficiently large $\rho$. We let $\rho_{k}$ denote the value of $\rho$ returned by solving (\ref{eq:alternating-descent-1}). The procedure terminates if $\rho_{k} \leq 0$ or if $|\rho_{k} - \rho_{k-1}^{\prime}| < \epsilon$. Otherwise, we solve the SOS problem with variables $\rho$ and $b^{k}$ given by

\begin{equation}
\label{eq:alternating-descent-2}
\begin{array}{ll}
\mbox{minimize} & \rho \\
\mbox{s.t.} & \alpha^{k}(x)\frac{\partial b^{k}}{\partial x}f(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)\left[\frac{\partial b^{k}}{\partial x}g(x)\right]_{i}} \\
& + \eta^{k}(x)b^{k}(x) + \rho\Lambda(x)-1 \in SOS \\
& -\beta^{k}(x)b^{k}(x) + w(x)h(x) - 1 \in SOS 
\end{array}
\end{equation}
We let $\rho_{k}^{\prime}$ denote the value of $\rho$ returned by the optimization. The procedure terminates if $\rho \leq 0$ or if $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$. The following theorem establishes correctness of this approach.
\begin{theorem}
\label{theorem:alternating-descent-CBF}
If the procedure described above terminates at stage $k$ with $\rho_{k} \leq 0$, then $b^{k-1}(x)$ is a CBF and $\{b^{k-1}(x) \geq 0\}$ is controlled positive invariant. If the procedure terminates at stage $k$ with $\rho_{k}^{\prime} \leq 0$, then $b^{k}(x)$ is a CBF and $\{b^{k}(x) \geq 0\}$ is controlled positive invariant. The procedure converges in a finite number of iterations.
\end{theorem}
\begin{proof}
We will show that if $\rho_{k} \leq 0$, then $b^{k-1}(x)$ is a CBF and $\{b^{k-1}(x) \geq 0\}$ is controlled positive invariant. If $\rho_{k} \leq 0$, then by construction of (\ref{eq:alternating-descent-1}) there exist SOS polynomials $\bar{\alpha}(x)$ and $\bar{\beta}(x)$ such that
\begin{IEEEeqnarray}{rCl}
\nonumber
\overline{\alpha}(x) &=& \alpha^{k}(x)\frac{\partial b^{k-1}}{\partial x}f(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)\left[\frac{\partial b^{k-1}}{\partial x}g(x)\right]_{i}} \\
\label{eq:alternating-descent-proof-1}
&& +\eta^{k}(x)b^{k-1}(x) + \rho_{i}\Lambda(x) - 1\\
\label{eq:alternating-descent-proof-2}
\overline{\beta}(x) &=& -\beta^{k}(x)b^{k-1}(x) + w(x)h(x) - 1
\end{IEEEeqnarray}
Rearranging (\ref{eq:alternating-descent-proof-1}) and setting $\overline{\theta} = -\theta_{i}^{k}$ and $\overline{\eta} = -\eta^{k}$ yields
\begin{multline*}
\sum_{i=1}^{m}{\overline{\theta}_{i}(x)\left[\frac{\partial b^{k-1}}{\partial x}g(x)\right]_{i}} + \overline{\eta}(x)b^{k-1}(x) \\
+ \overline{\alpha}(x) - \rho_{k}\Lambda(x) - \alpha^{k}(x)\frac{\partial b^{k-1}}{\partial x}f(x) + 1 = 0
\end{multline*}
Since $\rho_{k} \leq 0$ and $\Lambda(x)$ is SOS, $\overline{\alpha}(x) - \rho_{k}\Lambda(x)$ is SOS. Hence, by Theorem \ref{theorem:CBF-verification}, there does not exist any $x$ satisfying $$\frac{\partial b^{k-1}}{\partial x}f(x) \leq 0, \ b^{k-1}(x) = 0, \ \frac{\partial b^{k-1}}{\partial x}g(x) = 0$$ and $b^{k-1}(x)$ is a CBF by Theorem \ref{theorem:CBF-verification}. The case where $\rho_{k}^{\prime} \leq 0$ is similar.

To prove convergence, we observe that $\rho_{k-1}^{\prime}$, $\alpha^{k-1}(x)$, $\eta^{k-1}(x)$, $\theta_{1}^{k-1}(x),\ldots,\theta_{m}^{k-1}(x)$, and $\beta^{k-1}(x)$ comprise a feasible solution to (\ref{eq:alternating-descent-1}) and $\rho_{k}$, $b^{k-1}(x)$ are feasible solutions to (\ref{eq:alternating-descent-2}). Hence $\rho_{1} \geq \rho_{1}^{\prime} \geq \cdots \geq \rho_{k} \geq \rho_{k}^{\prime} \geq \cdots$, i.e., the sequence is monotone nonincreasing. If the sequence is unbounded, then there exists $K$ such that $\rho_{k}, \rho_{k}^{\prime} \leq 0$ for all $k > K$, and hence the algorithm terminates after $K$ iterations. If the sequence is bounded below by zero, then it converges by the monotone convergence theorem and hence $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$ and $|\rho_{k} - \rho_{k-1}^{\prime}| < \epsilon$ for $k$ sufficiently large.
\end{proof}

We next consider synthesis of HOCBFs. We initialize functions $b^{0}(x),\psi_{0}^{0}(x),\ldots,\psi_{r}^{0}(x)$ arbitrarily. We initialize parameters $\rho_{0}$ and $\rho_{0}^{\prime}$ to be infinite. We then solve an SOS problem with variables $\rho$, $\eta^{k}(x)$, $\theta_{1}^{k}(x),\ldots,\theta_{m}^{k}(x)$, $\{\lambda_{S}(x) : S \subseteq \{0,\ldots,r+1\}\}$, $\{\beta_{S}^{k}(x) : S \subseteq \{0,\ldots,r\}\}$, and $w^{k}(x)$ under two constraints. The first constraint ensures CPI and is given by
\begin{multline}
\label{eq:alternating-HOCBF-constraint-1}
\rho\Lambda(x) + \eta^{k}(x)\psi_{r}^{k-1}(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)L_{f}^{r-1}b^{k-1}(x)} \\
 + \sum_{S  \subseteq \{0,\ldots,(r+1)\}}{\left[\lambda_{S}(x)(L_{f}^{r}b(x) + O(b(x)))\right.} \\
 \cdot \left.\prod_{l \in S}{\psi_{l}^{k}(x)}\right] 
  + (L_{f}^{r}b(x) + O(b(x)))^{2s} \in SOS
  \end{multline}
The second constraint ensures containment within the safe region and is given by
\begin{multline}
\label{eq:alternating-HOCBF-constraint-2}
\sum_{S  \subseteq \{0,\ldots,r\}}{\beta_{S}^{k}(x)\prod_{l \in S}{\psi_{l}^{k-1}(x)}} + w^{k}(x)h(x) + 1 \in SOS
\end{multline}
Hence the overall SOS program can be stated as
\begin{equation}
\label{eq:alternating-descent-HOCBF-1}
\begin{array}{ll}
\mbox{minimize} & \rho \\
\mbox{s.t.} &  (\ref{eq:alternating-HOCBF-constraint-1}), (\ref{eq:alternating-HOCBF-constraint-2}) \\
 & \lambda_{S}^{k}(x), \beta_{S}^{k}(x) \in SOS
 \end{array}
 \end{equation}

 

We let $\rho_{k}$ denote the value of $\rho$ returned by solving (\ref{eq:alternating-descent-HOCBF-1}). The procedure terminates if $\rho_{k} \leq 0$ or if $|\rho_{k}-\rho_{k-1}^{\prime}| < \epsilon$. Otherwise, the algorithm proceeds by solving the SOS problem with variables $\rho$, $b^{k}$, and $\psi_{0}^{k},\ldots,\psi_{r}^{k}$ and constraints
\begin{multline}
\label{eq:alternating-HOCBF-constraint-3}
\rho\Lambda(x) + \eta^{k}\psi_{r}^{k}(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)L_{f}^{r-1}b^{k}(x)} \\
  + \sum_{S  \subseteq \{0,\ldots,(r+1)\}}{\lambda_{S}(x)(L_{f}^{r}b^{k}(x) + O(b^{k}(x)))}\\
  \cdot \prod_{l \in S}{\psi_{l}^{k}(x)} \in SOS
  \end{multline}
  and
  \begin{multline}
  \label{eq:alternating-HOCBF-constraint-4}
\sum_{S  \subseteq \{0,\ldots,r\}}{\beta_{S}^{k}(x)\prod_{l \in S}{\psi_{l}^{k-1}(x)}} + w^{k}(x)h(x) + 1 \in SOS
\end{multline}
The SOS program is stated as
 \begin{equation}
 \label{eq:alternating-descent-HOCBF-2}
 \begin{array}{ll}
 \mbox{minimize} & \rho \\
 \mbox{s.t.} &  (\ref{eq:alternating-HOCBF-constraint-3}), (\ref{eq:alternating-HOCBF-constraint-4})
 \end{array}
 \end{equation}
 The procedure terminates if $\rho^{\prime} \leq 0$ or if $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$. Similar to Theorem \ref{theorem:alternating-descent-CBF}, it can be shown that this approach terminates within finite time, and returns an HOCBF if $\rho \leq 0$ or $\rho^{\prime} \leq 0$ at convergence.
 
 \subsection{CBF Computation at Fixed Points}
 \label{subsec:fixed-points}
 We next describe how structures such as the existence of fixed points and periodic orbits in trajectories can be leveraged to construct CBFs. We first consider the case where the system $\dot{x}(t) = f(x) + g(x)u$ has a fixed point $(x^{\ast},u^{\ast})$, and have the following result.
 
 \begin{lemma}
 \label{lemma:fixed-point}
 Suppose that (\ref{eq:dynamics}) is controllable and $(x^{\ast},u^{\ast})$ is a fixed point. Then there exists $\epsilon > 0$ and a positive definite matrix $P$ such that $b(x) = \epsilon - (x-x^{\ast})^{T}P(x-x^{\ast})$ is a CBF.
 \end{lemma}
 
 \begin{proof}
 Let $\dot{x}(t) = Fx(t) + Gu(t)$ be the linearization of (\ref{eq:dynamics}) in a neighborhood of $(x^{\ast},u^{\ast})$. Let $\tilde{u}(t) = u^{\ast}-K(x-x^{\ast})$ be a stabilizing controller of the linearized system. Then there is a quadratic Lyapunov function $V(x) = (x-x^{\ast})^{T}P(x-x^{\ast})$ such that (\ref{eq:dynamics}) is asymptotically stable in a neighborhood of $x^{\ast}$, i.e., $$\frac{\partial V}{\partial x}(f(x) + g(x)\tilde{u}(t)) \leq 0.$$ This is equivalent to $\frac{\partial b}{\partial x}(f(x) + g(x)\tilde{u}) \geq 0$ for $(x-x^{\ast})$ sufficiently small. 
 \end{proof}
 
 The preceding lemma implies that we can construct a CBF by computing a fixed point $(x^{\ast},u^{\ast})$ and a stabilizing linear controller $\overline{u} = -K\overline{x}$ of the linearized system and solving the Lyapunov equation $\overline{F}^{T}P + P\overline{F} + N = 0$ where $\overline{F} = (F-GK)$ and $N$ is a positive definite matrix. It remains to choose the parameter $\epsilon$, which can be performed via the following procedure.
 
 \begin{theorem}
 \label{theorem:fixed-point}
 Suppose that $(x^{\ast},u^{\ast})$ is a fixed point of (\ref{eq:dynamics}), $P$ is a solution to the Lyapunov equation for a stabilizing controller of the linearized sytsem at $(x^{\ast},u^{\ast})$, and the SOS constraints
 \begin{multline}
 \label{eq:fixed-point-1}
 \alpha(x)(-2(x-x^{\ast})^{T}Pf(x)) + \sum_{i=1}^{m}{\theta_{i}(x)[-2(x-x^{\ast})^{T}Pg(x)]_{i}} \\
 + \eta(x)(\epsilon - (x-x^{\ast})^{T}P(x-x^{\ast})) \in SOS
 \end{multline}
 and
 \begin{equation}
 \label{eq:fixed-point-2}
 h(x)-\beta(x)(\epsilon - (x-x^{\ast})^{T}P(x-x^{\ast})) \in SOS
 \end{equation}
 hold for some polynomials $\theta_{1},\ldots,\theta_{m}$, $\eta(x)$ and SOS polynomials $\alpha(x)$ and $\beta(x)$. Then $b(x) = \epsilon - (x-x^{\ast})^{T}P(x-x^{\ast}))$ is a CBF and $\{b(x) \geq 0\}$ is in the safe region.
 \end{theorem}
 
 \begin{proof}
 If (\ref{eq:fixed-point-1}) holds, then $b$ is a CBF by Theorem \ref{theorem:CBF-verification}. By nonnegativity of SOS polynomials, we have that $b(x) \geq 0$ implies $h(x) \geq 0$ if $h(x) = \beta(x)b(x) + \beta_{0}(x)$ for SOS polynomials $\beta$ and $\beta_{0}$. Rearranging terms gives (\ref{eq:fixed-point-2}).
 \end{proof}

 \subsection{Newton's Method-Based Approach}
 \label{subsec:Newton}
 In what follows, we describe a method for synthesizing a single CBF to satisfy a safety constraint $\mathcal{B} = \{x: h(x) \geq 0\}$. We assume that $\mathcal{B}$ is compact, and later discuss how relaxing this assumption to general $\mathcal{B}$ affects the results. Our approach is to compute polynomials $b$, $\eta$, $\theta_{1},\ldots,\theta_{m}$, $w$, $\alpha_{01},\ldots,\alpha_{0N}$, $\beta_{01},\ldots,\beta_{0N}$, $\alpha_{11},\ldots,\alpha_{1N}$, $\beta_{11},\ldots,\beta_{1N}$ that solve the equations
 \begin{IEEEeqnarray}{rCl}
 \label{eq:Newton-1}
 \eta b + \sum_{i=1}^{m}{\theta_{i}\frac{\partial b}{\partial x}g_{i}} + \sum_{i=1}^{N}{\alpha_{0i}^{2}} - \sum_{i=1}^{N}{\alpha_{1i}^{2}\frac{\partial b}{\partial x}f} + 1 &=& 0 \IEEEeqnarraynumspace \\
 \label{eq:Newton-2}
 \sum_{i=1}^{N}{\beta_{1i}^{2}}b + wh + \sum_{i=1}^{N}{\beta_{0i}^{2}} + 1 &=& 0
 \end{IEEEeqnarray}
 These equations correspond to the conditions (\ref{eq:CBF-verification-1}) and (\ref{eq:HOCBF-verification-2}) in the special case where there is no $x$ with $b(x) = 0$, $\frac{\partial b}{\partial x}g(x) = 0$, and $\frac{\partial b}{\partial x}f(x) \leq  0$. 

 Our approach to solving the system is to use Newton's method  over function space. Define the function $F: X \rightarrow Y$, where $X = (\mathcal{C}^{1}(\mathcal{B})) \times (\mathcal{C}^{0}(\mathcal{B}))^{4N+m+2}$ and $Y = \mathcal{C}^{0}(\mathcal{B}) \times \mathcal{C}^{1}(\mathcal{B})$,  and $F = (F_{1} \ F_{2})^{T}$ is given by  
 \begin{IEEEeqnarray*}{rCl}
 F_{1} &=& \eta b + \sum_{i=1}^{m}{\theta_{i}\frac{\partial b}{\partial x}g_{i}} + \sum_{i=1}^{N}{\alpha_{0i}^{2}} - \sum_{i=1}^{N}{\alpha_{1i}^{2}} + 1 \\
F_{2} &=& \sum_{i=1}^{N}{\beta_{1i}^{2}}b + w(x)h(x) + \sum_{i=1}^{N}{\beta_{0i}^{2}} + 1
\end{IEEEeqnarray*}
In what follows, we let $\alpha_{0} = \sum_{i=1}^{N}{\alpha_{0i}^{2}}$, $\alpha_{1} = \sum_{i=1}^{N}{\alpha_{1i}^{2}}$, $\beta_{0} = \sum_{i=1}^{N}{\beta_{0i}^{2}}$, and $\beta_{1} = \sum_{i=1}^{N}{\beta_{1i}^{2}}$.  
Here $\mathcal{C}^{0}(\mathcal{B})$ denotes the set of continuous functions on $\mathcal{B}$ and $\mathcal{C}^{1}(\mathcal{B})$ denotes the set of continuously differentiable functions on $\mathcal{B}$.

The space $X$ is equipped with the sup-norm $$||\zeta||_{X}= \max{\left\{||\zeta_{1}||_{\infty}^{\mathcal{B}} + \big|\big|\frac{\partial \zeta_{1}}{\partial x}\big|\big|_{\infty}^{\mathcal{B}}, \max_{i \in \{2,\ldots,4N+m+2\}}{||\zeta_{i}||_{\infty}^{\mathcal{B}}}\right\}},$$ where $$||\zeta_{i}||_{\infty}^{\mathcal{B}} = \sup_{x \in \mathcal{B}}{|\zeta_{i}(x)|}.$$ while $Y$ is equipped with the norm $$||\chi||_{Y} = \max{\{||\chi_{1}||_{\infty}^{\mathcal{B}}, ||\chi_{2}||_{\infty}^{\mathcal{B}} + \big|\big|\frac{\partial \chi_{2}}{\partial x}\big|\big|_{\infty}^{\mathcal{B}}\}}.$$ We recall that the Frechet derivative of a function $F$ between Banach spaces $X$ and $Y$ is a bounded linear operator $A: X \rightarrow Y$ satisfying
\begin{equation}
\label{eq:Frechet-def}
\lim_{||\chi|| \rightarrow 0}{\frac{||F(\zeta + \chi) - F(\zeta) - A\chi||_{Y}}{||\chi||_{X}}} = 0.
\end{equation}
We have the following initial result. As a notation, we let $0^{l}$ denote the a vector of $l$ $0$'s.
\begin{lemma}
\label{lemma:Frechet}
The Frechet derivative of $F$ defined above is given by
\begin{equation}
\label{eq:Frechet}
    F^{\prime}(\zeta) = \left(
    \begin{array}{c}
    F_{11}(\zeta) \quad F_{12}(\zeta) \\
    F_{2}(\zeta)
    \end{array}
    \right)
\end{equation}
    with $$F_{11} = \eta + \sum_{i=1}^{m}{\theta_{i}\sum_{j=1}^{n}{g_{ij}D_{j}}} - \alpha_{1}\sum_{j=1}^{n}{f_{j}D_{j}}$$ 
    and
    \begin{IEEEeqnarray*}{rCl}
    \IEEEeqnarraymulticol{3}{l}{
    F_{12}} \\
    &=&
    \left(b \ \frac{\partial b}{\partial x}g_{1} \ \cdots \ \frac{\partial b}{\partial x}g_{m} \ 0 \ (2\alpha_{0i}: i=1,\ldots,N)  \right.\\
    && \quad \left. (-2\alpha_{1i}\frac{\partial b}{\partial x}f(x) : i=1,\ldots,N) \ 0^{2N}\right) \\
    \IEEEeqnarraymulticol{3}{l}{
    F_{22}} \\
    &=& \left(\beta_{1} \ 0^{m+1} \ h \ 0^{2N} \ (2\beta_{0i} : i=1,\ldots,N) \right. \\ 
    && \left. \quad (2\beta_{1i}b : i=1,\ldots,N)\right)
    \end{IEEEeqnarray*}
where $D_{j}$ denotes the differentiation operator $\frac{\partial b}{\partial x_{j}}$, i.e., differentiation of the first element of $\zeta$ with respect to $x_{j}$. 
\end{lemma}

\begin{proof}
The fact that (\ref{eq:Frechet}) is linear and satisfies (\ref{eq:Frechet-def}) is clear. It remains to show that $F^{\prime}(\zeta)$ is bounded, and it suffices to show that each entry of (\ref{eq:Frechet}) is bounded. For the top-left entry, we have 
\begin{IEEEeqnarray*}{rCl}
\IEEEeqnarraymulticol{3}{l}{
||\eta b+ \sum_{i=1}^{m}{\theta_{i}\sum_{j=1}^{n}{g_{ij}D_{j}b}} - \alpha_{1}\sum_{j=1}^{n}{f_{j}D_{j}b}||_{\infty}^{\mathcal{B}}
} \\
&\leq & ||\eta||_{\infty}^{\mathcal{B}}||b||_{\infty}^{\mathcal{B}} + \sum_{i=1}^{m}{\sum_{j=1}^{n}{||\theta_{i}g_{ij}||_{\infty}^{\mathcal{B}}||D_{j}b||_{\infty}^{\mathcal{B}}}} \\
&& + ||\alpha_{1}||_{\infty}^{\mathcal{B}}\sum_{j=1}^{n}{||f_{j}||_{\infty}^{\mathcal{B}}||D_{j}b||_{\infty}^{\mathcal{B}}} \\
&\leq& \left(||\eta||_{\infty}^{\mathcal{B}} + \sum_{i=1}^{m}{\sum_{j=1}^{n}{||\theta_{i}g_{ij}||_{\infty}^{\mathcal{B}}}} + ||\alpha_{1}||_{\infty}^{\mathcal{B}}\sum_{j=1}^{n}{||f_{j}||_{\infty}^{\mathcal{B}}}\right)||b||_{X}
\end{IEEEeqnarray*}
where the last inequality follows from the fact that 
\begin{IEEEeqnarray*}{rCl}
||b||_{\infty}^{\mathcal{B}} &\leq& ||b||_{\infty}^{\mathcal{B}} + \sum_{j=1}^{n}{||D_{j}b||_{\infty}^{\mathcal{B}}} \\
||D_{j}b||_{\infty}^{\mathcal{B}} &\leq & ||b||_{\infty}^{\mathcal{B}} + \sum_{j=1}^{n}{||D_{j}b||_{\infty}^{\mathcal{B}}}
\end{IEEEeqnarray*}
The remaining entries consist of multiplying by functions that are bounded on $\mathcal{B}$ and hence are bounded linear operators.
\end{proof}

Within this framework, solving (\ref{eq:Newton-1}) and (\ref{eq:Newton-2}) is equivalent to solving an underdetermined system of nonlinear equations in function space. The Newton's method procedure for solving such systems is as follows \cite{polyak2006newton}. First, define 
\begin{multline*}
\zeta^{k} = (b^{k}, \eta^{k}, (\theta_{i}^{k} : i=1,\ldots,N), w^{k}, \\
(\alpha_{ij}^{k} : i=0,1, j=1,\ldots,N), (\beta_{ij}^{k} : i=0,1, j=1,\ldots,N))^{T}
\end{multline*}
and select a parameter $\mu > 0$. After initializing $\zeta^{0}$, $\zeta^{k}$ is updated at each iteration as $\zeta^{k+1} = \zeta^{k}-\phi^{k}$, where $\phi^{k}$ is a solution to 
\begin{equation}
\label{eq:Newton-step}
F^{\prime}(\zeta^{k})\phi^{k} = F(\zeta^{k}), \ ||\phi^{k}||_{X} \leq \mu ||F(\zeta^{k})||_{Y}
\end{equation}
and $F^{\prime}(\zeta^{k})$ is the Frechet derivative of $F$ at $\zeta^{k}$. 
The following preliminary result gives sufficient conditions for Newton's method to converge to a solution  of an underdetermined nonlinear system.

\begin{theorem}[\cite{polyak2006newton},Theorem 3]
\label{theorem:Newtons-sufficient-general}
Suppose that $F: X \rightarrow Y$ is defined and differentiable on a ball $B=\{||\zeta_{0}-\zeta||_X \leq r\}$ and the following conditions hold:
\begin{enumerate}
\item There exists $L \geq 0$ such that $||F^{\prime}(\zeta)-F^{\prime}(\zeta^{\prime})||_{X,Y} \leq L||\zeta-\zeta^{\prime}||_{X}$ for all $\zeta,\zeta^{\prime} \in B$.
%\item For all $\zeta \in B$, $F^{\prime}(\zeta)$ maps $X$ onto $Y$.
\item There exists $\mu > 0$ such that $||F^{\prime}(\zeta)^{\ast}y|| \geq \mu||y||$ for all $\zeta \in B$ and $y \in Y^{\ast}$, where $^{\ast}$ denotes the dual.
\end{enumerate}
Define $$H_{n}(t) = \sum_{k=n}^{\infty}{t^{2^{k}}}$$ and suppose that 
\begin{displaymath}
\xi = \frac{L\mu^{2}||F(\zeta^{0})||}{2} < 1, \quad \rho = \frac{2H_{0}(\xi)}{L\mu} \leq r
\end{displaymath}
Then the update rule (\ref{eq:Newton-step}) converges to a solution $\zeta^{\ast}$ of $F(\zeta) = 0$, $||\zeta^{\ast} - \zeta^{0}|| \leq \rho$, with the rate $$||\zeta^{k}-\zeta^{\ast}|| \leq \frac{2H_{k}(\xi)}{L\mu}.$$
\end{theorem}
We will show that conditions 1) and 2) of Theorem \ref{theorem:Newtons-sufficient-general} are satisfied, and hence our approach guarantees local convergence. 
%As a notation, define the set $S_{\epsilon}(\phi_{1},\ldots,\phi_{M})$ for a collection of polynomials $\phi_{1},\ldots,\phi_{M}$ as $$S_{\epsilon} = \bigcap_{i=1}^{M}{\{x : |\phi_{i}(x)| < \epsilon\}}.$$

We first give a sequence of preliminary results before stating and proving the main convergence result.

\begin{lemma}
\label{lemma:Newton-Lipschitz}
For any $\zeta^{\ast}$ such that $F(\zeta^{\ast}) = 0$, there exist $L \geq 0$ and $\epsilon > 0$ such that $||F^{\prime}(\zeta) - F^{\prime}(\zeta^{\prime})||_{X,Y} \leq L||\zeta-\zeta^{\prime}||_{X}$ for all $\zeta,\zeta^{\prime} \in B(\zeta^{\ast},\epsilon)$. 
\end{lemma}

\begin{proof}
It suffices to show that each entry of $F^{\prime}(\zeta)$ satisfies a Lipschitz condition for some $L \geq 0$. This is equivalent to showing that there exists $L$ such that, for any $\zeta_{1},\zeta_{2}, \overline{\zeta} \in X$, we have $$||(F^{\prime}(\zeta_{1})-F^{\prime}(\zeta_{2}))\overline{\zeta}||_{Y} \leq L||\zeta_{1}-\zeta_{2}||_{X}||\overline{\zeta}||_{X}.$$  Considering $F_{11}^{\prime}$ first, we have 
\begin{IEEEeqnarray*}{rCl}
\IEEEeqnarraymulticol{3}{l}{
||(\eta_{1}-\eta_{2} + \sum_{i=1}^{m}{(\theta_{i}^{1}-\theta_{i}^{2})\sum_{j=1}^{n}{g_{ij}D_{j}}} - (\alpha^{1}-\alpha^{2})\sum_{j=1}^{n}{f_{j}D_{j}})\overline{\zeta}||_{X}} \\
&\leq& ||(\eta_{1}-\eta_{2})\overline{\zeta}||_{Y} + \sum_{i=1}^{m}{||(\theta_{i}^{1}-\theta_{i}^{2})\sum_{j=1}^{n}{g_{ij}D_{j}\overline{\zeta}}||_{Y}} \\
&& + ||(\alpha_{1}^{1}-\alpha_{1}^{2})\sum_{j=1}^{n}{f_{j}D_{j}\overline{\zeta}}||_{Y} \\
&\leq& ||\eta_{1}-\eta_{2}||_{Y}||\overline{\zeta}||_{Y} + \sum_{i=1}^{m}{\sum_{j=1}^{n}{||(\theta_{i}^{1}-\theta_{i}^{2})\sum_{j=1}^{n}{g_{ij}}||||D_{j}\overline{\zeta}||_{Y}}} \\
&& + ||\alpha_1^{1}-\alpha_1^{2}||_{Y}\sum_{j=1}^{n}{||f_{j}||_{Y}||D_{j}\overline{\zeta}||_{Y}}
\end{IEEEeqnarray*}
by basic properties of the norm, where $\eta^{1}$, $\eta^{2}$, and the remaining polynomials denote the corresponding entries of $\zeta_{1}$ and $\zeta_{2}$. Now, we have that $||\overline{\zeta}||_{Y} \leq ||\overline{\zeta}||_{X}$ and $||D_{j}\overline{\zeta}||_{Y} \leq ||\overline{\zeta}||_{X}$. Hence 
\begin{multline*}
||(F^{\prime}(\zeta_{1})-F^{\prime}(\zeta_{2}))\overline{\zeta}|| \\
\leq \left(||\eta_{1}-\eta_{2}||_{Y} + ||\sum_{i=1}^{m}{\sum_{j=1}^{n}{||(\theta_{i}^{1}-\theta_{i}^{2})g_{ij}}}||_{Y}  \right. \\
 \left. + ||\alpha_{1}^{1}-\alpha_{1}^{2}||_{Y}\sum_{j=1}^{n}{||f_{j}||_{Y}}||\overline{\zeta}||_{X}\right)||\overline{\zeta}||_{X}
\end{multline*}
Implying that the Lipschitz property holds. The remaining entries are linear functions of the polynomials in $\zeta_{1}$ and $\zeta_{2}$, and hence the local Lipschitz property holds for those entries as well.
\end{proof}

The following known result states that the set of bounded and surjective linear operators is open.

\begin{lemma}[\cite{rudinfunctional}]
\label{lemma:Newton-intermediate-1}
Let $G: X \rightarrow Y$ be a surjective and bounded linear operator between two Banach spaces $X$ and $Y$. Then there exists $\epsilon > 0$ such that any bounded linear operator $G^{\prime}: X \rightarrow Y$ with $||G-G^{\prime}||_{X,Y} < \epsilon$ is surjective. 
\end{lemma}

We next give a sufficient condition for $F^{\prime}(\zeta)$ to be surjective.
\begin{lemma}
\label{lemma:Newton-intermediate-2}
Suppose that $F_{12}^{\prime}(\zeta)$ and $F_{2}^{\prime}(\zeta)$ are surjective. Then $F^{\prime}(\zeta)$ is surjective.
\end{lemma}

\begin{proof}
Suppose that $F_{12}^{\prime}(\zeta)$ and $F_{2}^{\prime}(\zeta)$ are surjective. Let $y = (y_{1} \ y_{2})^{T}$. We construct $\overline{\zeta}$ such that $F^{\prime}(\zeta)\overline{\zeta} = y$ as follows. First, select $\overline{\zeta}$ such that $\overline{b}$, $\overline{\omega}$, $\overline{\beta}_{11},\ldots,\overline{\beta}_{1N}$, and $\overline{\beta}_{01},\ldots,\overline{\beta}_{0N}$  satisfy $F_{2}^{\prime}(\zeta)\overline{\zeta} =y_{2}$ when all other entries of $\overline{\zeta}$ are 0.  Next, let $$\hat{y}_{1} = y_{1} - \left(\eta \overline{b} + \sum_{i=1}^{m}{\theta_{i}\frac{\partial \overline{b}}{\partial x}g_{i}} - \alpha_{1} \frac{\partial \overline{b}}{\partial x}f\right),$$ and choose $\overline{\eta}$, $\overline{\theta}_{1},\ldots,\overline{\theta}_{m}$, and $(\overline{\alpha}_{ij}: i=0,1,j=1,\ldots,N)$ such that $$F_{12}^{\prime}(\zeta)\left(
\begin{array}{c}
\overline{\eta} \\
\overline{\theta}_{1} \\
\vdots \\
\overline{\theta}_{m} \\
0 \\
\overline{\alpha}_{01} \\
\vdots \\
\overline{\alpha}_{1N} \\
\vdots
\end{array}
\right) = \hat{y}_{1}.$$
Combining these choices for the entries of $\overline{\zeta}$ yields $\overline{\zeta}$ with $F^{\prime}(\zeta)\overline{\zeta} = y$.
\end{proof}

Next, we leverage this result to prove that $F^{\prime}(\zeta)$ is surjective in a neighborhood of $\zeta^{\ast}$.

\begin{lemma}
\label{lemma:Newton-intermediate-3}
Suppose that $\zeta^{\ast}$ is a solution to $F(\zeta) = 0$. Then there exists $\epsilon > 0$ such that $||\zeta-\zeta^{\ast}||_{XY} < \epsilon$ implies that $F^{\prime}(\zeta)$ is surjective.
\end{lemma}

\begin{proof}
We first show that $F^{\prime}(\zeta^{\ast})$ is surjective. By Lemma \ref{lemma:Newton-intermediate-2}, it suffices to show that $F_{12}^{\prime}(\zeta^{\ast})$ and $F_{2}^{\prime}(\zeta^{\ast})$ are surjective. We first consider $F_{12}^{\prime}(\zeta^{\ast})$, and suppose $y_{1} \in \mathcal{C}^{0}(\mathcal{B})$ is given. Since $\zeta^{\ast}$ is a solution to (\ref{eq:Newton-1}), we have that $$\eta^{\ast}b^{\ast} + \sum_{i=1}^{m}{\theta_{i}^{\ast}\frac{\partial b^{\ast}}{\partial x}g_{i}}- \sum_{i=1}^{N}{\frac{\partial b^{\ast}}{\partial x}f(x)\alpha_{1i}^{2}} + \sum_{i=1}^{N}{\alpha_{0i}^{2}} = -1.$$ Choosing $\bar{\eta} = -y_{1}\eta^{\ast}$, $\bar{\theta}_{i} = -\bar{\theta}^{\ast}y_{1}$, $\bar{\alpha}_{i0} = -\frac{1}{2}y_{1}\alpha_{i0}^{\ast}$, and $\bar{\alpha}_{i1} = -\frac{1}{2}y_{1}\alpha_{i1}^{\ast}\frac{\partial b^{\ast}}{\partial x}f(x)$ gives the desired result.

We next turn to $F_{2}^{\prime}(\zeta^{\ast})$. Since $\zeta^{\ast}$ is a solution to (\ref{eq:Newton-2}), we have that $$\sum_{i=1}^{N}{\beta_{1i}^{2}b^{\ast}} + w^{\ast}h + \sum_{i=1}^{N}{\beta_{0i}^{2}} = -1.$$ We can therefore choose $\overline{b} = 0$, $\overline{\beta}_{1i} = -\frac{1}{2}y_{2}b^{\ast}\beta_{1i}$, $\overline{w} = -y_{2}h$, and $\overline{\beta}_{0i} = -\frac{1}{2}y_{2}\overline{\beta}_{0i}$ to ensure that $F_{2}^{\prime}(\zeta^{\ast})\overline{\zeta} = y_{2}$.

Now, since the norms of each entry of $F_{12}^{\prime}$ and $F_{2}^{\prime}$ are bounded, we have that $F_{12}^{\prime}$ and $F_{2}^{\prime}$ are bounded linear operators, and hence by Lemma \ref{lemma:Newton-intermediate-1}, there exists $\epsilon$ such that any bounded linear operator $G$ with $||G-F_{12}^{\prime}(\zeta^{\ast})|| < \epsilon$ or $||G-F_{2}^{\prime}(\zeta^{\ast})|| < \epsilon$ is surjective. Hence by Lemma \ref{lemma:Newton-Lipschitz}, $F_{12}(\zeta)$ and $F_{2}(\zeta)$ are surjective for any $\zeta$ sufficiently close to $\zeta^{\ast}$. Finally, by Lemma \ref{lemma:Newton-intermediate-2}, we have that $F^{\prime}(\zeta)$ is surjective for $\zeta$ sufficiently close to $\zeta^{\ast}$. 
\end{proof}

We are now ready to state the main convergence result.

\begin{theorem}
\label{theorem:Newton-convergence}
There exist parameters $r$, $L$, and $\mu$ such that, if $||\zeta^{0}-\zeta^{\ast}|| \leq r$, where $\zeta^{\ast}$ is a polynomial solution to $F(\zeta) = 0$, then the Newton update rule (\ref{eq:Newton-step}) converges to a fixed point $\hat{\zeta}$ of $F$ with rate given in Theorem \ref{theorem:Newtons-sufficient-general}.
\end{theorem}


\begin{proof}
The approach of the proof is to show that the conditions of Theorem \ref{theorem:Newtons-sufficient-general} are satisfied. Conditions 1 follows from Lemma \ref{lemma:Newton-Lipschitz}. By \cite[Theorem 4.13]{rudinfunctional}, Condition 2 holds if $F^{\prime}(\zeta)$ is surjective for all $\zeta$ in  a neighborhood of $\zeta^{\ast}$. Hence Condition 2 holds by Lemma \ref{lemma:Newton-intermediate-3}. 
%Condition 2 follows from Lemma \ref{lemma:Newton-intermediate-3} and \textbf{*ref Rudin, Theorem 4.13}.
%\emph{\underline{Proof of Condition 2):}} The goal is to find $\overline{\zeta}$ such that 
%\begin{displaymath}
%\left(
%\begin{array}{c}
%F_{1}^{\prime}(\zeta) \\
%F_{2}^{\prime}(\zeta)
%\end{array}
%\right)\overline{\zeta} = \left(
%\begin{array}{c}
%\overline{F}_{1} \\
%\overline{F}_{2}
%\end{array}
%\right).
%\end{displaymath}
%We first consider $F_{2}^{\prime}(\zeta)\overline{\zeta} = \overline{F}_{2}$. By Lemma \textbf{*ref} and condition 3), it suffices to prove the result for any polynomial $\zeta$. The goal is to find $\overline{b}$, $\overline{h}$, $\overline{\beta}_{11},\ldots,\overline{\beta}_{1N}$, $\overline{\beta}_{01},\ldots,\overline{\beta}_{0N}$ such that 
%\begin{equation}
%\label{eq:onto-1}
%\beta_{1}\overline{b} + h\overline{w} + 2\sum_{i=1}^{N}{\beta_{1i}b\overline{\beta}_{1i}} + 2\sum_{i=1}^{N}{\beta_{0i}\overline{\beta}_{0i}} = \overline{F}_{2}.
%\end{equation}
%By Lemma \textbf{*ref}, if $||\zeta-\zeta^{\ast}|| \leq \epsilon$ where $\zeta^{\ast}$ is a polynomial solution to $F(\zeta) = 0$, there exist polynomials $\phi_{1},\ldots,\phi_{N+2}$ such that $$\beta_{1}\phi_{1} + h\phi_{2} + \sum_{i=1}^{N}{\beta_{0i}\phi_{i+2}} = 1.$$ Choosing $\overline{\beta}_{1i} = 0$, $\overline{b} = \overline{F}_{2}\phi_{1}$, $\overline{w} = \overline{F}_{2}\phi_{2}$, and $\overline{\beta}_{0i} = \frac{1}{2}\overline{F}_{2}\phi_{i+2}$ then gives (\ref{eq:onto-1}). 
%Next, consider $F_{1}^{\prime}(\zeta)\overline{\zeta} = \overline{F}_{1}$. Let $$\hat{F}_{1} = \overline{F}_{1} - (\eta \overline{b} + \sum_{i=1}^{m}{\theta_{i}\frac{\partial \overline{b}}{\partial x}g_{i}} - \alpha_{1}\frac{\partial \overline{b}}{\partial x}f).$$ The goal is to find $$\overline{\eta}, \overline{\theta}_{1},\ldots, \overline{\theta}_{m}, \bar{\alpha}_{01},\ldots,\bar{\alpha}_{0N}, \bar{\alpha}_{11},\ldots,\bar{\alpha}_{1N}$$ such that
%\begin{equation}
%\label{eq:onto-2}
%b\overline{\eta} + \sum_{i=1}^{m}{\frac{\partial b}{\partial x}g_{i}\overline{\theta}_{i}} - 2\sum_{i=1}^{N}{\alpha_{1i}\frac{\partial b}{\partial x}f(x)\overline{\alpha}_{1i}}+2\sum_{i=1}^{N}{\alpha_{0i}\bar{\alpha}_{0i}} = \hat{F}_{1}
%\end{equation}
%By Lemma \textbf{*ref}, there exist functions $\psi_{1},\ldots,\psi_{2N+m+2}$ such that 
%\begin{multline*}
%b\psi_{1} + \sum_{i=1}^{m}{\frac{\partial b}{\partial x}g_{i}\psi_{i+1}} + \sum_{i=1}^{N}{\alpha_{1i}\frac{\partial b}{\partial x}f(x)\psi_{m+1+i}} \\
%+ \sum_{i=1}^{N}{\alpha_{0i}\psi_{N+m+1+i}} = 1
%\end{multline*}
%Hence, if we choose $\overline{\eta} = \psi_{1}\hat{F}_{1}$, $\overline{\theta}_{i} = \psi_{i+1}\hat{F}_{1}$, $\overline{\alpha}_{1i} = -\frac{1}{2}\psi_{m+1+i}\hat{F}_{1}$, $\overline{\alpha}_{0i} = -\frac{1}{2}\psi_{N+m+1+i}\hat{F}_{1}$, we obtain (\ref{eq:onto-2}).
%for $(y_{1} \ y_{2}) \in Y^{\ast}$, we have 
%\begin{IEEEeqnarray*}{rCl}
%\IEEEeqnarraymulticol{3}{l}{
%||F^{\prime}(x^{\ast})y|| 
%} \\
%&=& \sup_{\stackrel{\gamma_{1},\ldots,\gamma_{4N+m+3}}{||\gamma_{i}|| \leq 1}}{\left\{\int{y_{1}(x)(\eta + \sum_{i=1}^{m}{\theta_{i}\sum_{j=1}^{n}{g_{ij}D_{j}}}-\alpha_{1}\sum_{j=1}^{n}{f_{j}D_{j}})\gamma_{1} \ dx}\right.} \\
%&& + \int{y_{2}(x)\beta_{1}(x)\gamma_{1}(x) \ dx} \\
%&& + \int{y_{1}(x)b(x)\gamma_{2}(x) \ dx} + \sum_{i=1}^{m}{\int{y_{1}\frac{\partial b}{\partial x}g_{i}(x)\gamma_{i+1}(x) \ dx}} \\
%&& -\sum_{i=1}^{N}{\int{y_{1}(x)(2\alpha_{0i}(x)\gamma_{m+i+1}(x) \ dx}} \\
%&& + \sum_{i=1}^{N}{\int{y_{1}(x)(2\alpha_{1i}(x))\frac{\partial b}{\partial x}f(x)\gamma_{N+m+1+i}(x) \ dx}} \\
%&& + \int_{y_{2}(x)h(x)\gamma_{2N+m+2}(x) \ dx} + \sum_{i=1}^{N}{\int{\gamma_{2}(x)(2\beta_{0i}(x)\gamma_{2N+m+2+i}(x) \ dx}} \\
%&& + \sum_{i=1}^{N}{\int{y_{2}(x)(2\beta_{1i}(x)b(x)\gamma_{3N+m+2+i}(x) \ dx}}
%\end{IEEEeqnarray*}
%If $||y_{1}||=||y_{2}|| = 1$, then in order to have $||F^{\prime}(x)^{\ast}y|| < \epsilon$, we need $$\mbox{supp}(y_{1}) \subseteq \left(\{|b(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{m}{\{|\frac{\partial b}{\partial x}g_{i}| < \epsilon\}}\right) \cap \{|\frac{\partial b}{\partial x}f| < \epsilon\} \cap \left(\bigcap_{i=1}^{N}{\{|\alpha_{0i}(x)| < \epsilon\}}\right)\right) \cup \left(\{|b(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{m}{\{|\frac{\partial b}{\partial x}g_{i}| < \epsilon\}}\right) \cap \left(\bigcap_{i=1}^{N}{\{|\alpha_{1i}(x)| < \epsilon\}}\right) \cap \left(\bigcap_{i=1}^{N}{\{|\alpha_{0i}(x)| < \epsilon\}}\right)\right).$$ However, by Lemma \textbf{*ref}, this set is empty. Alternatively, we could choose $y_{1} = 0$ and $$\mbox{supp}(y_{2}) \subseteq \left(\{|b(x)| < \epsilon\} \cap \{|h(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{N}{\{|\beta_{0i}(x)| < \epsilon\}}\right)\right) \cup \left(\{|h(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{N}{\{|\beta_{0i}(x)| < \epsilon\}}\right) \cap \left(\bigcap_{i=1}^{N}{\{|\beta_{1i}(x)| < \epsilon\}}\right)\right).$$ However, these sets are also empty by Lemma \textbf{*ref}. This argument can be extended to a neighborhood of $\zeta^{\ast}$ via continuity of $F^{\ast}$.
\end{proof}

Theorem \ref{theorem:Newton-convergence} implies that the Newton's algorithm procedure converges at a quadratic rate to a fixed point $b$ that satisfies (\ref{eq:Newton-1}) and (\ref{eq:Newton-2}), provided that the initial $b_{0}$ is sufficiently close to a solution. While there is no guarantee that $b$ is a polynomial function, we note that any such solution can be used as a CBF. First, $b$ is continuously differentiable. We have that, if $h(x) = 0$, then $\beta_{1}(x)b(x) + \beta_{0}(x) + 1= 0$ for some SOS functions $\beta_{0}$ and $\beta_{1}$, implying that $b(x) < 0$, implying that the controlled positive invariant set defined by $b$ is contained in $\mathcal{C}$. Furthermore, if $b(x) = 0$ and $\frac{\partial b}{\partial x}g(x) = 0$ for all $x$, then $-\alpha_{1}(x)\frac{\partial b}{\partial x}f(x) + \alpha_{0}(x) + 1 = 0$, implying that $\frac{\partial b}{\partial x}f(x) > 0$. 

We next remark on the case where $\mathcal{C}$ is not compact. In order to ensure that the norm is well-defined, we can define $X$ and $Y$ over a different compact set, e.g., the ball in $\mathbb{R}^{n}$ of radius 1. If the Newton's method procedure converges to a smooth function such as a polynomial, then (\ref{eq:Newton-1}) and (\ref{eq:Newton-2}) are guaranteed to hold over all of $\mathbb{R}^{n}$, implying that $b$ is a CBF. However, there is no guarantee that the limit point of the procedure will satisfy this condition.

==> Synthesis.tex <==
\section{Problem Formulation: CBF Synthesis}
\label{sec:synthesis}
This section presents two approaches to synthesizing CBFs.

\subsection{Alternating Descent Approach}
\label{subsec:ad-synthesis}
Our first approach is based on the SOS constraints introduced in Section \ref{sec:verification}. When the function $b(x)$ is unknown, the constraints become nonlinear and non-convex. We therefore propose an alternating-descent heuristic, in which we alternate between updating the CBF candidate $b(x)$ and the polynomials used for verification. We describe our approach for synthesizing CBFs for polynomial dynamics, although a similar approach can be used to construct an intersection of CBFs (based on Section \textbf{*ref}), HOCBFs, and CBFs involving Lagrangian or trigonometric functions.

We initialize a function $b^{0}(x)$ arbitrarily (e.g., $b^{0}(x) = h_{i}(x)$ for some $i$) and initialize parameters $\rho_{0}$ and $\rho_{0}^{\prime}$ to be infinite. At step $k$, we solve the following SOS program with variables $\rho$, $\alpha^{k}(x)$, $\eta^{k}(x)$, $\theta_{1}^{k}(x),\ldots,\theta_{m}^{k}(x)$, $w(x)$, and $\beta^{k}(x)$:

\begin{equation}
\label{eq:alternating-descent-1}
\begin{array}{ll}
\mbox{minimize} & \rho \\
\mbox{s.t.} & \alpha^{k}(x)\frac{\partial b^{k-1}}{\partial x}f(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)\left[\frac{\partial b^{k-1}}{\partial x}g(x)\right]_{i}} \\
& + \eta^{k}(x)b^{k-1}(x) + \rho \Lambda(x) - 1 \in SOS \\
& -\beta^{k}(x)b^{k-1}(x) + w(x)h(x) - 1 \in SOS \\
& \beta^{k}(x), \alpha^{k}(x) \in SOS
\end{array}
\end{equation}

In (\ref{eq:alternating-descent-1}), $\Lambda(x)$ is an SOS polynomial chosen to ensure that the first constraint is SOS for sufficiently large $\rho$. We let $\rho_{k}$ denote the value of $\rho$ returned by solving (\ref{eq:alternating-descent-1}). The procedure terminates if $\rho_{k} \leq 0$ or if $|\rho_{k} - \rho_{k-1}^{\prime}| < \epsilon$. Otherwise, we solve the SOS problem with variables $\rho$ and $b^{k}$ given by

\begin{equation}
\label{eq:alternating-descent-2}
\begin{array}{ll}
\mbox{minimize} & \rho \\
\mbox{s.t.} & \alpha^{k}(x)\frac{\partial b^{k}}{\partial x}f(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)\left[\frac{\partial b^{k}}{\partial x}g(x)\right]_{i}} \\
& + \eta^{k}(x)b^{k}(x) + \rho\Lambda(x)-1 \in SOS \\
& -\beta^{k}(x)b^{k}(x) + w(x)h(x) - 1 \in SOS 
\end{array}
\end{equation}
We let $\rho_{k}^{\prime}$ denote the value of $\rho$ returned by the optimization. The procedure terminates if $\rho \leq 0$ or if $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$. The following theorem establishes correctness of this approach.
\begin{theorem}
\label{theorem:alternating-descent-CBF}
If the procedure described above terminates at stage $k$ with $\rho_{k} \leq 0$, then $b^{k-1}(x)$ is a CBF and $\{b^{k-1}(x) \geq 0\}$ is controlled positive invariant. If the procedure terminates at stage $k$ with $\rho_{k}^{\prime} \leq 0$, then $b^{k}(x)$ is a CBF and $\{b^{k}(x) \geq 0\}$ is controlled positive invariant. The procedure converges in a finite number of iterations.
\end{theorem}
\begin{proof}
We will show that if $\rho_{k} \leq 0$, then $b^{k-1}(x)$ is a CBF and $\{b^{k-1}(x) \geq 0\}$ is controlled positive invariant. If $\rho_{k} \leq 0$, then by construction of (\ref{eq:alternating-descent-1}) there exist SOS polynomials $\bar{\alpha}(x)$ and $\bar{\beta}(x)$ such that
\begin{IEEEeqnarray}{rCl}
\nonumber
\overline{\alpha}(x) &=& \alpha^{k}(x)\frac{\partial b^{k-1}}{\partial x}f(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)\left[\frac{\partial b^{k-1}}{\partial x}g(x)\right]_{i}} \\
\label{eq:alternating-descent-proof-1}
&& +\eta^{k}(x)b^{k-1}(x) + \rho_{i}\Lambda(x) - 1\\
\label{eq:alternating-descent-proof-2}
\overline{\beta}(x) &=& -\beta^{k}(x)b^{k-1}(x) + w(x)h(x) - 1
\end{IEEEeqnarray}
Rearranging (\ref{eq:alternating-descent-proof-1}) and setting $\overline{\theta} = -\theta_{i}^{k}$ and $\overline{\eta} = -\eta^{k}$ yields
\begin{multline*}
\sum_{i=1}^{m}{\overline{\theta}_{i}(x)\left[\frac{\partial b^{k-1}}{\partial x}g(x)\right]_{i}} + \overline{\eta}(x)b^{k-1}(x) \\
+ \overline{\alpha}(x) - \rho_{k}\Lambda(x) - \alpha^{k}(x)\frac{\partial b^{k-1}}{\partial x}f(x) + 1 = 0
\end{multline*}
Since $\rho_{k} \leq 0$ and $\Lambda(x)$ is SOS, $\overline{\alpha}(x) - \rho_{k}\Lambda(x)$ is SOS. Hence, by Theorem \ref{theorem:CBF-verification}, there does not exist any $x$ satisfying $$\frac{\partial b^{k-1}}{\partial x}f(x) \leq 0, \ b^{k-1}(x) = 0, \ \frac{\partial b^{k-1}}{\partial x}g(x) = 0$$ and $b^{k-1}(x)$ is a CBF by Theorem \ref{theorem:CBF-verification}. The case where $\rho_{k}^{\prime} \leq 0$ is similar.

To prove convergence, we observe that $\rho_{k-1}^{\prime}$, $\alpha^{k-1}(x)$, $\eta^{k-1}(x)$, $\theta_{1}^{k-1}(x),\ldots,\theta_{m}^{k-1}(x)$, and $\beta^{k-1}(x)$ comprise a feasible solution to (\ref{eq:alternating-descent-1}) and $\rho_{k}$, $b^{k-1}(x)$ are feasible solutions to (\ref{eq:alternating-descent-2}). Hence $\rho_{1} \geq \rho_{1}^{\prime} \geq \cdots \geq \rho_{k} \geq \rho_{k}^{\prime} \geq \cdots$, i.e., the sequence is monotone nonincreasing. If the sequence is unbounded, then there exists $K$ such that $\rho_{k}, \rho_{k}^{\prime} \leq 0$ for all $k > K$, and hence the algorithm terminates after $K$ iterations. If the sequence is bounded below by zero, then it converges by the monotone convergence theorem and hence $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$ and $|\rho_{k} - \rho_{k-1}^{\prime}| < \epsilon$ for $k$ sufficiently large.
\end{proof}

We next consider synthesis of HOCBFs. We initialize functions $b^{0}(x),\psi_{0}^{0}(x),\ldots,\psi_{r}^{0}(x)$ arbitrarily. We initialize parameters $\rho_{0}$ and $\rho_{0}^{\prime}$ to be infinite. We then solve the SOS problem with variables $\rho$, $\eta^{k}(x)$, $\theta_{1}^{k}(x),\ldots,\theta_{m}^{k}(x)$, $\{\lambda_{S}(x) : S \subseteq \{0,\ldots,r+1\}\}$, $\{\beta_{S}^{k}(x) : S \subseteq \{0,\ldots,r\}\}$, and $w^{k}(x)$ given by 

\begin{equation}
\label{eq:alternating-descent-HOCBF-1}
\begin{array}{ll}
\mbox{minimize} & \rho \\
\mbox{s.t.} & \rho\Lambda(x) + \eta^{k}(x)\psi_{r}^{k-1}(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)L_{f}^{r-1}b^{k-1}(x)} + \sum_{S \in \subseteq \{0,\ldots,(r+1)\}}{\lambda_{S}(x)(L_{f}^{r}b(x) + O(b(x)))\prod_{l \in S}{\psi_{l}^{k}(x)}} \\
 & + (L_{f}^{r}b(x) + O(b(x)))^{2s} \in SOS \\
 & \sum_{S \in \subseteq \{0,\ldots,r\}}{\beta_{S}^{k}(x)\prod_{l \in S}{\psi_{l}^{k-1}(x)}} + w^{k}(x)h(x) + 1 \in SOS \\
 & \lambda_{S}^{k}(x), \beta_{S}^{k}(x) \in SOS
 \end{array}
 \end{equation}
 We let $\rho_{k}$ denote the value of $\rho$ returned by solving (\ref{eq:alternating-descent-HOCBF-1}). The procedure terminates if $\rho_{k} \leq 0$ or if $|\rho_{k}-\rho_{k-1}^{\prime}| < \epsilon$. Otherwise, the algorithm proceeds by solving the SOS problem with variables $\rho$, $b^{k}$, and $\psi_{0}^{k},\ldots,\psi_{r}^{k}$ given by
 \begin{equation}
 \label{eq:alternating-descent-HOCBF-2}
 \begin{array}{ll}
 \mbox{minimize} & \rho \\
 \mbox{s.t.} & \rho\Lambda(x) + \eta^{k}\psi_{r}^{k}(x) + \sum_{i=1}^{m}{\theta_{i}^{k}(x)L_{f}^{r-1}b^{k}(x)} \\
 & + \sum_{S \in \subseteq \{0,\ldots,(r+1)\}}{\lambda_{S}(x)(L_{f}^{r}b^{k}(x) + O(b^{k}(x)))\prod_{l \in S}{\psi_{l}^{k}(x)}} \in SOS
 \sum_{S \in \subseteq \{0,\ldots,r\}}{\beta_{S}^{k}(x)\prod_{l \in S}{\psi_{l}^{k-1}(x)}} + w^{k}(x)h(x) + 1 \in SOS
 \end{array}
 \end{equation}
 The procedure terminates if $\rho^{\prime} \leq 0$ or if $|\rho_{k}-\rho_{k}^{\prime}| < \epsilon$. Similar to Theorem \ref{theorem:alternating-descent-CBF}, it can be shown that this approach terminates within finite time, and returns an HOCBF if $\rho \leq 0$ or $\rho^{\prime} \leq 0$ at convergence.
 
 \subsection{CBF Computation at Fixed Points}
 \label{subsec:fixed-points}
 We next describe how structures such as the existence of fixed points  in trajectories can be leveraged to construct CBFs. We first consider the case where the system $\dot{x}(t) = f(x) + g(x)u$ has a fixed point $(x^{\ast},u^{\ast})$, and have the following result.
 
 \begin{lemma}
 \label{lemma:fixed-point}
 Suppose that (\ref{eq:dynamics}) is controllable and $(x^{\ast},u^{\ast})$ is a fixed point. Then there exists $\epsilon > 0$ and a positive definite matrix $P$ such that $b(x) = \epsilon - (x-x^{\ast})^{T}P(x-x^{\ast})$ is a CBF.
 \end{lemma}
 
 \begin{proof}
 Let $\dot{x}(t) = Fx(t) + Gu(t)$ be the linearization of (\ref{eq:dynamics}) in a neighborhood of $(x^{\ast},u^{\ast})$. Let $\tilde{u}(t) = u^{\ast}-K(x-x^{\ast})$ be a stabilizing controller of the linearized system. Then there is a quadratic Lyapunov function $V(x) = (x-x^{\ast})^{T}P(x-x^{\ast})$ such that (\ref{eq:dynamics}) is asymptotically stable in a neighborhood of $x^{\ast}$, i.e., $$\frac{\partial V}{\partial x}(f(x) + g(x)\tilde{u}(t)) \leq 0.$$ This is equivalent to $\frac{\partial b}{\partial x}(f(x) + g(x)\tilde{u}) \geq 0$ for $(x-x^{\ast})$ sufficiently small. 
 \end{proof}
 
 The preceding lemma implies that we can construct a CBF by computing a fixed point $(x^{\ast},u^{\ast})$ and a stabilizing linear controller $\overline{u} = -K\overline{x}$ of the linearized system and solving the Lyapunov equation $\overline{F}^{T}P + P\overline{F} + N = 0$ where $\overline{F} = (F-GK)$ and $N$ is a positive definite matrix. It remains to choose the parameter $\epsilon$, which can be performed via the following procedure.
 
 \begin{theorem}
 \label{theorem:fixed-point}
 Suppose that $(x^{\ast},u^{\ast})$ is a fixed point of (\ref{eq:dynamics}), $P$ is a solution to the Lyapunov equation for a stabilizing controller of the linearized sytsem at $(x^{\ast},u^{\ast})$, and the SOS constraints
 \begin{multline}
 \label{eq:fixed-point-1}
 \alpha(x)(-2(x-x^{\ast})^{T}Pf(x)) + \sum_{i=1}^{m}{\theta_{i}(x)[-2(x-x^{\ast})^{T}Pg(x)]_{i}} \\
 + \eta(x)(\epsilon - (x-x^{\ast})^{T}P(x-x^{\ast})) \in SOS
 \end{multline}
 and
 \begin{equation}
 \label{eq:fixed-point-2}
 h(x)-\beta(x)(\epsilon - (x-x^{\ast})^{T}P(x-x^{\ast})) \in SOS
 \end{equation}
 hold for some polynomials $\theta_{1},\ldots,\theta_{m}$, $\eta(x)$ and SOS polynomials $\alpha(x)$ and $\beta(x)$. Then $b(x) = \epsilon - (x-x^{\ast})^{T}P(x-x^{\ast}))$ is a CBF and $\{b(x) \geq 0\}$ is in the safe region.
 \end{theorem}
 
 \begin{proof}
 If (\ref{eq:fixed-point-1}) holds, then $b$ is a CBF by Theorem \ref{theorem:CBF-verification}. By nonnegativity of SOS polynomials, we have that $b(x) \geq 0$ implies $h(x) \geq 0$ if $h(x) = \beta(x)b(x) + \beta_{0}(x)$ for SOS polynomials $\beta$ and $\beta_{0}$. Rearranging terms gives (\ref{eq:fixed-point-2}).
 \end{proof}

 \subsection{Newton's Method-Based Approach}
 \label{subsec:Newton}
 In what follows, we describe a method for synthesizing a single CBF to satisfy a safety constraint $\mathcal{C} = \{x: h(x) \geq 0\}$. Our approach is to compute polynomials $b$, $\eta$, $\theta_{1},\ldots,\theta_{m}$, $\alpha_{01},\ldots,\alpha_{0N}$, $\beta_{01},\ldots,\beta_{0N}$, $\alpha_{11},\ldots,\alpha_{1N}$, $\beta_{11},\ldots,\beta_{1N}$ that solve the equations
 \begin{IEEEeqnarray}{rCl}
 \label{eq:Newton-1}
 \eta b + \sum_{i=1}^{m}{\theta_{i}\frac{\partial b}{\partial x}g_{i}} + \sum_{i=1}^{N}{\alpha_{0i}^{2}} - \sum_{i=1}^{N}{\alpha_{1i}^{2}\frac{\partial b}{\partial x}f(x)} + 1 &=& 0 \\
 \label{eq:Newton-2}
 \sum_{i=1}^{N}{\beta_{1i}^{2}}b + w(x)h(x) + \sum_{i=1}^{N}{\beta_{0i}^{2}} + 1 &=& 0
 \end{IEEEeqnarray}
 These equations correspond to the conditions (\ref{eq:CBF-verification-1}) and (\ref{eq:HOCBF-verification-2}) in the special case where there is no $x$ with $\frac{\partial b}{\partial x}f(x) = 0$. 

 Our approach to solving the system is to use a Newton's method approach over function space. Define the function $F: X \rightarrow Y$, where $X = (\mathcal{C}^{1})^{4N+m+3}$, $Y = \mathcal{C}^{2}$, and $F = (F_{1} \ F_{2})^{T}$ where 
 \begin{IEEEeqnarray*}{rCl}
 F_{1} &=& \eta b + \sum_{i=1}^{m}{\theta_{i}\frac{\partial b}{\partial x}g_{i}} + \sum_{i=1}^{N}{\alpha_{0i}^{2}} - \sum_{i=1}^{N}{\alpha_{1i}^{2}} + 1 \\
F_{2} &=& \sum_{i=1}^{N}{\beta_{1i}^{2}}b + w(x)h(x) + \sum_{i=1}^{N}{\beta_{0i}^{2}} + 1
\end{IEEEeqnarray*}
The space $X$ is equipped with the sup-norm $$||\zeta||_{X} =\sup_{i=1,\ldots,4N+m+2}{||\zeta_{i}||_{\infty} + ||\frac{\partial \zeta_{i}}{\partial x}||_{\infty}},$$ while $Y$ is equipped with the sup-norm $$||\chi||_{Y} = \sup_{i=1,2}{||\chi_{i}||_{\infty}}.$$ 

Within this framework, solving (\ref{eq:Newton-1}) and (\ref{eq:Newton-2}) is equivalent to solving an underdetermined system of nonlinear equations in function space. The Newton's method procedure for solving such systems is as follows \textbf{*ref}. First, define $$\zeta^{k} = (b^{k}, \eta^{k}, (\theta_{i}^{k} : i=1,\ldots,N), w^{k}, (\alpha_{ij}^{k} : i=0,1, j=1,\ldots,N), (\beta_{ij}^{k} : i=0,1, j=1,\ldots,N))$$ and select a parameter $\mu > 0$. After initializing $\zeta^{0}$, $\zeta^{k}$ is updated at each iteration as $\zeta^{k+1} = \zeta^{k}-\phi^{k}$, where $\phi^{k}$ is a solution to 
\begin{equation}
\label{eq:Newton-step}
F^{\prime}(\zeta^{k})\phi^{k} = F(\zeta^{k}), \ ||\phi^{k}||_{X} \leq \mu ||F(\zeta^{k})||_{Y}
\end{equation}
and $F^{\prime}(\zeta^{k})$ is the Frechet derivative of $F$ at $\zeta^{k}$. The Frechet derivative $F^{\prime}(\zeta^{k})$ is given by
\begin{multline}
\label{eq:Frechet}
    F^{\prime}(\zeta^{k}) = \\
    \left(
    \begin{array}{cccccccccccccccccc}
    \left(\eta + \sum_{i=1}^{m}{\theta_{i}\sum_{j=1}^{n}{g_{ij}D_{j}}} - \alpha_{1}\sum_{j=1}^{n}{f_{j}D_{j}}\right) \ b & \frac{\partial b}{\partial x}g_{1} & \cdots & \frac{\partial b}{\partial x}g_{m} & 0 & 2\alpha_{01} & \cdots & 2\alpha_{0N} & -2\alpha_{10}\frac{\partial b}{\partial x}f(x) & \cdots & -2\alpha_{1N}\frac{\partial b}{\partial x}f(x) & 0 & \cdots & 0 & 0 & \cdots & 0 \\
    \beta_{1} & 0 & 0 & \cdots & 0 & h & 0 & \cdots & 0 & 0 &\cdots & 0 & 2\beta_{01} & \cdots & 2\beta_{0N} & 2\beta_{11}b & \cdots & 2\beta_{1N}b
    \end{array}
    \right)
\end{multline}
where $D_{j}$ denotes the differentiation operator $\frac{\partial b}{\partial x_{j}}$, i.e., differentiation of the first element of $\zeta$ with respect to $x_{j}$. The following preliminary result gives sufficient conditions for Newton's method to converge to a solution to a fixed point of an underdetermined nonlinear system.

\begin{theorem}[\textbf{*ref}]
\label{theorem:Newtons-sufficient-general}
Suppose that $F: X \rightarrow Y$ is defined and differentiable on a ball $B=\{||\zeta_{0}-\zeta||_X \leq r\}$ and the following conditions hold:
\begin{enumerate}
\item There exists $L \geq 0$ such that $||F^{\prime}(\zeta)-F^{\prime}(\zeta^{\prime})|| \leq L||\zeta-\zeta^{\prime}||_{X}$ for all $\zeta,\zeta^{\prime} \in B$.
%\item For all $\zeta \in B$, $F^{\prime}(\zeta)$ maps $X$ onto $Y$.
\item There exists $\mu > 0$ such that $||F^{\prime}(\zeta)^{\ast}y|| \geq \mu||y||$ for all $\zeta \in B$ and $y \in Y^{\ast}$, where $^{\ast}$ denotes the dual.
\end{enumerate}
Define $$H_{n}(t) = \sum_{k=n}^{\infty}{t^{2^{k}}}$$ and suppose that 
\begin{displaymath}
h = \frac{L\mu^{2}||F(\zeta^{0})||}{2} < 1, \quad \rho = \frac{2H_{0}(h)}{L\mu} \leq r
\end{displaymath}
Then the update rule (\ref{eq:Newton-step}) converges to a solution $\zeta^{\ast}$ of $F(\zeta) = 0$, $||\zeta^{\ast} - \zeta^{0}|| \leq \rho$, with the rate $$||\zeta^{k}-\zeta^{\ast}|| \leq \frac{2H_{k}(h)}{L\mu}.$$
\end{theorem}
We will show that conditions 1)-3) of Theorem \ref{theorem:Newtons-sufficient-general} are satisfied, and hence our approach guarantees local convergence. We have the following initial result.
\begin{lemma}
\label{lemma:preliminary-Newton-result}
Let $\zeta^{\ast}$ be a polynomial solution to $F(\zeta^{\ast}) =0$, and let $\xi = (\eta \ \theta_{1} \ \ldots \theta_{m} \ w \ (\alpha_{ij}:i=0,1,j=1,\ldots,N) \ (\beta_{ij} : i=0,1,j=1,\ldots,N))$. Suppose that the polynomials in $\xi$ are indexed $\xi_{1},\ldots,4N+m+2$ Then the following conditions hold: \textbf{*fill this in later.}
\end{lemma}

As a notation, define the set $S_{\epsilon}(\phi_{1},\ldots,\phi_{M})$ for a collection of polynomials $\phi_{1},\ldots,\phi_{M}$ as $$S_{\epsilon} = \bigcap_{i=1}^{M}{\{x : |\phi_{i}(x)| < \epsilon\}}.$$

We are now ready to state the main convergence result.

\begin{theorem}
\label{theorem:Newton-convergence}
There exist parameters $r$, $L$, and $\mu$ such that, if $||\zeta^{0}-\zeta^{\ast}|| \leq r$, where $\zeta^{\ast}$ is a polynomial solution to $F(\zeta) = 0$, then the Newton update rule (\ref{eq:Newton-step}) converges to a fixed point $\hat{\zeta}$ of $F$ with rate given in \textbf{*ref}.
\end{theorem}

Before presenting the proof of Theorem \ref{theorem:Newton-convergence}, we provide an intermediate result.

\begin{lemma}
\label{lemma:Newton-intermediate-1}
Let $X$ and $Y$ be defined as above. Let $G_{i}: X \rightarrow Y$ be a sequence of continuous linear operators that converge uniformly to a continuous linear operator $G$. Let $y \in Y$ and suppose that, for all $i$, there exists $\zeta_{i}$ with $G_{i}\zeta_{i} = y$, where the $\zeta_{i}$ are uniformly bounded. Suppose further that there exists $\mu > 0$ such that $||G_{i}\zeta|| \geq \mu ||\zeta||$ for all $\zeta$. Then there exists $\overline{\zeta}$ satisfying $G\overline{\zeta} = y$.
\end{lemma}

\begin{proof}
For all $n,m$, we have that 
\begin{IEEEeqnarray*}{rCl}
0 &=& ||G_{n}\zeta_{n}-G_{m}\zeta_{m}|| \\
&=& ||G_{n}\zeta_{n}-G_{m}\zeta_{n}+G_{m}\zeta_{n}-G_{m}\zeta_{m}|| \\
&\geq& ||G_{m}\zeta_{n}-G_{m}\zeta_{m}|| - ||G_{n}\zeta_{n}-G_{m}\zeta_{n}|| 
\end{IEEEeqnarray*}
Rearranging terms gives 
\begin{IEEEeqnarray*}{rCl}
||G_{m}||||\zeta_{n}-\zeta_{m}|| &\leq& ||G_{m}(\zeta_{m}-\zeta_{n})|| \\
&\leq& ||G_{n}-G_{m}||||\zeta_{n}|| < \epsilon
\end{IEEEeqnarray*}
for $m,n$ sufficiently large
Hence $\zeta_{n}$ is a Cauchy sequence and converges to a limit $\overline{\zeta}$. Since $G_{i}\zeta_{i} = y$ for all $i$, we must then have $G\zeta = y$ as well.
\end{proof}



\begin{proof}[Proof of Theorem \ref{theorem:Newton-convergence}]
The approach of the proof is to show that the conditions of Theorem \ref{theorem:Newtons-sufficient-general} are satisfied.

\emph{\underline{Proof of Condition 1):}}  It suffices to show that each entry of $F^{\prime}(\zeta)$ satisfies a Lipschitz condition for some $L \geq 0$. This is equivalent to showing that there exists $L$ such that, for any $\zeta_{1},\zeta_{2}, \overline{\zeta} \in X$, we have $$||(F^{\prime}(\zeta_{1})-F^{\prime}(\zeta_{2}))\overline{\zeta}||_{Y} \leq L||\zeta_{1}-\zeta_{2}||_{X}||\overline{\zeta}||_{X}.$$ Let $(F^{\prime}(\zeta_{1})-F^{\prime}(\zeta_{2}))_{11}$ denote the upper-left entry of $(F^{\prime}(\zeta_{1})-F^{\prime}(\zeta_{2}))$. We have 
\begin{IEEEeqnarray*}{rCl}
\IEEEeqnarraymulticol{3}{l}{
||(\eta_{1}-\eta_{2} + \sum_{i=1}^{m}{(\theta_{i}^{1}-\theta_{i}^{2})\sum_{j=1}^{n}{g_{ij}D_{j}}} - (\alpha^{1}-\alpha^{2})\sum_{j=1}^{n}{f_{j}D_{j}})\overline{\zeta}||_{X}} \\
&\leq& ||(\eta_{1}-\eta_{2})||_{Y} + \sum_{i=1}^{m}{||(\theta_{i}^{1}-\theta_{i}^{2})\sum_{j=1}^{n}{g_{ij}D_{j}\overline{\zeta}}||_{Y}} + ||(\alpha_{1}^{1}-\alpha_{1}^{2})\sum_{j=1}^{n}{f_{j}D_{j}\overline{\zeta}}||_{Y} \\
&\leq& ||\eta_{1}-\eta_{2}||_{Y}||\overline{\zeta}||_{Y} + \sum_{i=1}^{m}{\sum_{j=1}^{n}{||(\theta_{i}^{1}-\theta_{i}^{2})\sum_{j=1}^{n}{g_{ij}}||||D_{j}\overline{\zeta}||_{Y}}} \\
&& + ||\alpha^{1}-\alpha^{2}||_{Y}\sum_{j=1}^{n}{||f_{j}||_{Y}||D_{j}\overline{\zeta}||_{Y}}
\end{IEEEeqnarray*}
by basic properties of the norm. Now, we have that $||\overline{\zeta}||_{Y} \leq ||\overline{\zeta}||_{X}$ and $||D_{j}\overline{\zeta}||_{Y} \leq ||\overline{\zeta}||_{X}$. Hence 
\begin{multline*}
||(F^{\prime}(\zeta_{1})-F^{\prime}(\zeta_{2}))\overline{\zeta}|| \\
\leq \left(||\eta_{1}-\eta_{2}||_{Y} + ||\sum_{i=1}^{m}{\sum_{j=1}^{n}{||(\theta_{i}^{1}-\theta_{i}^{2})g_{ij}}}||_{Y} + ||\alpha_{1}^{1}-\alpha_{1}^{2}||_{Y}\sum_{j=1}^{n}{||f_{j}||_{Y}}||\overline{\zeta}||_{X}\right)||\overline{\zeta}||_{X}
\end{multline*}
Implying that the Lipschitz property holds. The remaining entries are linear functions of the polynomials in $\zeta_{1}$ and $\zeta_{2}$, and hence the local Lipschitz property holds for those entries as well.

%\emph{\underline{Proof of Condition 2):}} The goal is to find $\overline{\zeta}$ such that 
%\begin{displaymath}
%\left(
%\begin{array}{c}
%F_{1}^{\prime}(\zeta) \\
%F_{2}^{\prime}(\zeta)
%\end{array}
%\right)\overline{\zeta} = \left(
%\begin{array}{c}
%\overline{F}_{1} \\
%\overline{F}_{2}
%\end{array}
%\right).
%\end{displaymath}
%We first consider $F_{2}^{\prime}(\zeta)\overline{\zeta} = \overline{F}_{2}$. By Lemma \textbf{*ref} and condition 3), it suffices to prove the result for any polynomial $\zeta$. The goal is to find $\overline{b}$, $\overline{h}$, $\overline{\beta}_{11},\ldots,\overline{\beta}_{1N}$, $\overline{\beta}_{01},\ldots,\overline{\beta}_{0N}$ such that 
%\begin{equation}
%\label{eq:onto-1}
%\beta_{1}\overline{b} + h\overline{w} + 2\sum_{i=1}^{N}{\beta_{1i}b\overline{\beta}_{1i}} + 2\sum_{i=1}^{N}{\beta_{0i}\overline{\beta}_{0i}} = \overline{F}_{2}.
%\end{equation}
%By Lemma \textbf{*ref}, if $||\zeta-\zeta^{\ast}|| \leq \epsilon$ where $\zeta^{\ast}$ is a polynomial solution to $F(\zeta) = 0$, there exist polynomials $\phi_{1},\ldots,\phi_{N+2}$ such that $$\beta_{1}\phi_{1} + h\phi_{2} + \sum_{i=1}^{N}{\beta_{0i}\phi_{i+2}} = 1.$$ Choosing $\overline{\beta}_{1i} = 0$, $\overline{b} = \overline{F}_{2}\phi_{1}$, $\overline{w} = \overline{F}_{2}\phi_{2}$, and $\overline{\beta}_{0i} = \frac{1}{2}\overline{F}_{2}\phi_{i+2}$ then gives (\ref{eq:onto-1}). 

%Next, consider $F_{1}^{\prime}(\zeta)\overline{\zeta} = \overline{F}_{1}$. Let $$\hat{F}_{1} = \overline{F}_{1} - (\eta \overline{b} + \sum_{i=1}^{m}{\theta_{i}\frac{\partial \overline{b}}{\partial x}g_{i}} - \alpha_{1}\frac{\partial \overline{b}}{\partial x}f).$$ The goal is to find $$\overline{\eta}, \overline{\theta}_{1},\ldots, \overline{\theta}_{m}, \bar{\alpha}_{01},\ldots,\bar{\alpha}_{0N}, \bar{\alpha}_{11},\ldots,\bar{\alpha}_{1N}$$ such that
%\begin{equation}
%\label{eq:onto-2}
%b\overline{\eta} + \sum_{i=1}^{m}{\frac{\partial b}{\partial x}g_{i}\overline{\theta}_{i}} - 2\sum_{i=1}^{N}{\alpha_{1i}\frac{\partial b}{\partial x}f(x)\overline{\alpha}_{1i}}+2\sum_{i=1}^{N}{\alpha_{0i}\bar{\alpha}_{0i}} = \hat{F}_{1}
%\end{equation}
%By Lemma \textbf{*ref}, there exist functions $\psi_{1},\ldots,\psi_{2N+m+2}$ such that 
%\begin{multline*}
%b\psi_{1} + \sum_{i=1}^{m}{\frac{\partial b}{\partial x}g_{i}\psi_{i+1}} + \sum_{i=1}^{N}{\alpha_{1i}\frac{\partial b}{\partial x}f(x)\psi_{m+1+i}} \\
%+ \sum_{i=1}^{N}{\alpha_{0i}\psi_{N+m+1+i}} = 1
%\end{multline*}
%Hence, if we choose $\overline{\eta} = \psi_{1}\hat{F}_{1}$, $\overline{\theta}_{i} = \psi_{i+1}\hat{F}_{1}$, $\overline{\alpha}_{1i} = -\frac{1}{2}\psi_{m+1+i}\hat{F}_{1}$, $\overline{\alpha}_{0i} = -\frac{1}{2}\psi_{N+m+1+i}\hat{F}_{1}$, we obtain (\ref{eq:onto-2}).

\emph{\underline{Proof of Condition 2):}} For $(y_{1} \ y_{2}) \in Y^{\ast}$, we have 
\begin{IEEEeqnarray*}{rCl}
\IEEEeqnarraymulticol{3}{l}{
||F^{\prime}(x^{\ast})y|| 
} \\
&=& \sup_{\stackrel{\gamma_{1},\ldots,\gamma_{4N+m+3}}{||\gamma_{i}|| \leq 1}}{\left\{\int{y_{1}(x)(\eta + \sum_{i=1}^{m}{\theta_{i}\sum_{j=1}^{n}{g_{ij}D_{j}}}-\alpha_{1}\sum_{j=1}^{n}{f_{j}D_{j}})\gamma_{1} \ dx}\right.} \\
&& + \int{y_{2}(x)\beta_{1}(x)\gamma_{1}(x) \ dx} \\
&& + \int{y_{1}(x)b(x)\gamma_{2}(x) \ dx} + \sum_{i=1}^{m}{\int{y_{1}\frac{\partial b}{\partial x}g_{i}(x)\gamma_{i+1}(x) \ dx}} \\
&& -\sum_{i=1}^{N}{\int{y_{1}(x)(2\alpha_{0i}(x)\gamma_{m+i+1}(x) \ dx}} \\
&& + \sum_{i=1}^{N}{\int{y_{1}(x)(2\alpha_{1i}(x))\frac{\partial b}{\partial x}f(x)\gamma_{N+m+1+i}(x) \ dx}} \\
&& + \int_{y_{2}(x)h(x)\gamma_{2N+m+2}(x) \ dx} + \sum_{i=1}^{N}{\int{\gamma_{2}(x)(2\beta_{0i}(x)\gamma_{2N+m+2+i}(x) \ dx}} \\
&& + \sum_{i=1}^{N}{\int{y_{2}(x)(2\beta_{1i}(x)b(x)\gamma_{3N+m+2+i}(x) \ dx}}
\end{IEEEeqnarray*}
If $||y_{1}||=||y_{2}|| = 1$, then in order to have $||F^{\prime}(x)^{\ast}y|| < \epsilon$, we need $$\mbox{supp}(y_{1}) \subseteq \left(\{|b(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{m}{\{|\frac{\partial b}{\partial x}g_{i}| < \epsilon\}}\right) \cap \{|\frac{\partial b}{\partial x}f| < \epsilon\} \cap \left(\bigcap_{i=1}^{N}{\{|\alpha_{0i}(x)| < \epsilon\}}\right)\right) \cup \left(\{|b(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{m}{\{|\frac{\partial b}{\partial x}g_{i}| < \epsilon\}}\right) \cap \left(\bigcap_{i=1}^{N}{\{|\alpha_{1i}(x)| < \epsilon\}}\right) \cap \left(\bigcap_{i=1}^{N}{\{|\alpha_{0i}(x)| < \epsilon\}}\right)\right).$$ However, by Lemma \textbf{*ref}, this set is empty. Alternatively, we could choose $y_{1} = 0$ and $$\mbox{supp}(y_{2}) \subseteq \left(\{|b(x)| < \epsilon\} \cap \{|h(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{N}{\{|\beta_{0i}(x)| < \epsilon\}}\right)\right) \cup \left(\{|h(x)| < \epsilon\} \cap \left(\bigcap_{i=1}^{N}{\{|\beta_{0i}(x)| < \epsilon\}}\right) \cap \left(\bigcap_{i=1}^{N}{\{|\beta_{1i}(x)| < \epsilon\}}\right)\right).$$ However, these sets are also empty by Lemma \textbf{*ref}. This argument can be extended to a neighborhood of $\zeta^{\ast}$ via continuity of $F^{\ast}$.
\end{proof}

==> Verification.tex <==
\section{Problem Formulation: CBF Verification}
\label{sec:verification}
This section presents our approach for CBF verification. We first give the problem statement and complexity results. We then formulate the problem of verifying CBFs as a sum-of-squares optimization. We generalize the verification problem to incorporate multiple CBFs, HOCBFs, dynamics with trigonometric functions, and actuation constraints.

\subsection{Problem Statement and Complexity Results}
\label{subsec:verification-statement}
The problem studied in this section is stated as follows.

\begin{problem}
\label{problem:verification}
Given a function $b: \mathbb{R}^{n} \rightarrow \mathbb{R}$, dynamics (\ref{eq:dynamics}), and a safety constraint $\mathcal{C}$, determine if $b$ is a CBF for safety constraint $\mathcal{C}$.
\end{problem}

The following initial result gives necessary and sufficient conditions for $b$ to be a CBF.

\begin{proposition}
\label{prop:CBF-conditions}
The function $b(x)$ is a CBF iff there is no $x$ satisfying $b(x) = 0$, $\frac{\partial b}{\partial x}g(x) = 0$, and $\frac{\partial b}{\partial x}f(x) < 0$.
\end{proposition}

\begin{proof}
By Nagumo's Theorem~\cite{aubin2011viability}, $b(x(t)) \geq 0$ for all $t \geq 0$ iff $\dot{b}(x(t)) \geq 0$ whenever $b(x(t)) = 0$. Suppose that $b(x) = 0$. If $\frac{\partial b}{\partial x}g(x) \neq 0$, then $u(t)$ can be chosen to satisfy (\ref{eq:CBF-def}). One such choice is to choose $i$ with $[\frac{\partial b}{\partial x}g(x)]_{i} \neq 0$, set $$u_{i}(t) = -\left(\left[\frac{\partial b}{\partial x}g(x)\right]_{i}\right)^{-1}(\frac{\partial b}{\partial x}f(x))$$ and $u_{j}(t) = 0$ for $j \neq i$. If $\frac{\partial b}{\partial x}g(x) = 0$ and $\frac{\partial b}{\partial x}f(x) \geq 0$, then $\dot{b}(x(t)) \geq 0$. 

Conversely, if $\frac{\partial b}{\partial x}g(x_{0}) = 0$, $b(x_{0}) = 0$, and $\frac{\partial b}{\partial x}f(x_{0}) < 0$ for some $x_{0}$, then the set $\{b(x) \geq 0\}$ is not positive invariant, since $x(t)$ will leave the set if $x(0) = x_{0}$.
\end{proof}

We observe that, in the statement of Problem 1, we do not require that the control policy is continuous, although we develop sufficient conditions for continuity in Proposition \ref{prop:smooth-safety}. We first consider the complexity of Problem \ref{problem:verification}. 
\begin{proposition}
\label{prop:CBF-complexity}
Problem \ref{problem:verification} is NP-hard.
\end{proposition}

\begin{proof}
NP-hardness of Problem \ref{problem:verification} is equivalent to NP-hardness of checking whether there exists $x$ satisfying the conditions of Proposition \ref{prop:CBF-conditions}. We will show that there exists a polynomial time reduction of the NP-hard problem of checking nonnegativity of a polynomial to the problem of verifying conditions of Proposition \ref{prop:CBF-conditions}. 

Let $r: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a polynomial. Define $b: \mathbb{R}^{n+1} \rightarrow \mathbb{R}$ by $b(x) = x_{n+1}r(x_{1},\ldots,x_{n})$ where $x = (x_{1},\ldots,x_{n},x_{n+1})^{T}$. Define $g: \mathbb{R}^{n+1} \rightarrow \mathbb{R}^{(n+1) \times m}$ by $g(x) \equiv 0$. Define $f: \mathbb{R}^{n+1} \rightarrow \mathbb{R}^{n+1}$ as $f(x) = (f_{1}(x),\ldots,f_{n+1}(x)^{T}$ with 
\begin{displaymath}
f_{i}(x) = \left\{
\begin{array}{ll}
0, & i \neq n+1 \\
1, & i = n+1
\end{array}
\right.
\end{displaymath}

We have that $\frac{\partial b}{\partial x}g(x) = 0$ and $\frac{\partial b}{\partial x}f(x) = \frac{\partial b}{\partial x_{n+1}}f_{n+1}(x) = r(x_{1},\ldots,x_{n})$. Suppose that there exists $x$ such that $b(x) = 0$ and $\frac{\partial b}{\partial x}f(x) < 0$. Then $x_{n+1}r(x_{1},\ldots,x_{n}) = 0$ and $r(x_{1},\ldots,x_{n}) < 0$, implying that $r$ is \emph{not} nonnegative. Conversely, if no such $x$ exists, then in particular there is no $(x_{1},\ldots,x_{n})^{T}$ with $b(x_{1},\ldots,x_{n},0) = 0$ and $\frac{\partial b}{\partial x}f(x) = r(x_{1},\ldots,x_{n}) < 0$, implying that $r$ is nonnegative. Hence $r$ is nonnegative if and only if $b$ is  CBF, implying NP-hardness of Problem \ref{problem:verification}.
\end{proof}

One heuristic approach to Problem \ref{problem:verification} is to search for a polynomial $\theta(x)$ such that 
\begin{equation}
\label{eq:verification-heuristic}
\frac{\partial b}{\partial x}(f(x) + g(x)\theta(x)) + \alpha(b(x))
\end{equation}
 is SOS \cite{ames2019control}. While this approach can be formulated as a convex optimization problem and gives a sufficient condition, it is not complete as shown by the following.

\begin{proposition}
\label{prop:CBF-complexity-negative}
There exist polynomials $b$, $f$, and $g$ such that $b$ is a CBF and, for any polynomial $\theta$ and class-K polynomial $\alpha$, (\ref{eq:verification-heuristic}) is not a sum-of-squares. 
\end{proposition}

\begin{proof}
Let $p: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a nonnegative polynomial that is not SOS. Define $b: \mathbb{R}^{n+1} \rightarrow \mathbb{R}$ as $b(x_{0},x) = x_{0}p(x)$. Define $f: \mathbb{R}^{n+1} \rightarrow \mathbb{R}^{n+1}$ and $g: \mathbb{R}^{n+1} \rightarrow \mathbb{R}^{(n+1) \times m}$ as $f(x_{0},x) = (1 \ 0 \ \cdots \ 0)^{T}$ and $g(x_{0},x) \equiv 0$.  By construction $\frac{\partial b}{\partial x}f(x) = p(x)$.

We first show that $b$ is a CBF. Suppose there is a point $x$ where $b(x) = 0$ and $\frac{\partial b}{\partial x}f(x) < 0$. Since $b(x_{0},x) = x_{0}p(x)$, we must have $x_{0} = 0$ or $p(x) = 0$. If $p(x) = 0$, then  $\frac{\partial b}{\partial x}f(x) = p(x) = 0$. If $x_{0} = 0$, then $\frac{\partial b}{\partial x}f(x) = p(x) \geq 0$. Hence $b$ is a CBF by Proposition \ref{prop:CBF-conditions}.

We next show that, for any polynomials $\alpha$ and $\theta$, (\ref{eq:verification-heuristic}) is not SOS. Suppose that, in fact, (\ref{eq:verification-heuristic}) is SOS. Since $\alpha$ is a class-K polynomial, $\alpha(0) = 0$ and hence $\alpha(z) = z\overline{\alpha}(z)$ for some polynomial $\overline{\alpha}: \mathbb{R} \rightarrow \mathbb{R}$. Hence (\ref{eq:verification-heuristic}) is equivalent to $$\psi(x,x_{0}) = p(x) + x_{0}p(x)\overline{\alpha}(x).$$ If $\psi(x,x_{0})$ is SOS, then $\overline{\psi}(x) = \psi(x,0)$ should also be SOS. Since $\psi(x,0) = p(x)$, this is a contradiction. Hence (\ref{eq:verification-heuristic}) is not SOS.
\end{proof}

We next give an equivalent condition for a function to be a CBF based on the Positivstellensatz.

\begin{theorem}
\label{theorem:CBF-verification}
A polynomial $b(x)$ is a CBF for (\ref{eq:dynamics}) if and only if there exist polynomials $\eta$, $\theta_{1},\ldots,\theta_{m}$, SOS polynomials $\alpha_{0}(x)$ and $\alpha_{1}(x)$, and an integer $r$ such that 
\begin{multline}
\label{eq:CBF-verification-1}
\eta(x)b(x) + \sum_{i=1}^{m}{\theta_{i}(x)\left[\frac{\partial b}{\partial x}g(x)\right]_{i}} \\
+\alpha_{0}(x) - \alpha_{1}(x)\frac{\partial b}{\partial x}f(x) \\
+ \left(\frac{\partial b}{\partial x} f(x)\right)^{2r} = 0
\end{multline}
Moreover, $x(t)$ remains in the safe region $\mathcal{C}$ under a CBF policy for $b$ if (\ref{eq:CBF-verification-1}) holds and there exist SOS polynomials $\beta_{0}(x)$ and $\beta_{1}(x)$ and a polynomial $\omega(x)$ such that 
\begin{equation}
\label{eq:CBF-verification-2}
\beta_{0}(x) + \beta_{1}(x)b(x) + \omega(x)h(x)+1 = 0
\end{equation}
\end{theorem}

\begin{proof}
By Proposition \ref{prop:CBF-conditions}, we have that $b(x)$ is a CBF iff there is no $x$ satisfying $b(x) = 0$, $\frac{\partial b}{\partial x}g(x) = 0$, and $\frac{\partial b}{\partial x}f(x) < 0$. The latter condition is equivalent to $-\frac{\partial b}{\partial x}f(x) \geq 0$ and $\frac{\partial b}{\partial x}f(x) \neq 0$. Furthermore, we have that $\Sigma[\frac{\partial b}{\partial x}f(x)]$ is equal to the set of polynomials of the form $\alpha_{0}(x) + \alpha_{1}(x)\frac{\partial b}{\partial x}f(x)$ where $\alpha_{0}$ and $\alpha_{1}$ are SOS. Hence the conditions of Proposition \ref{prop:CBF-conditions} are equivalent to (\ref{eq:CBF-verification-1}) by Theorem \ref{theorem:Psatz}.

Now, suppose that (\ref{eq:CBF-verification-1}), and hence $b(x(t)) \geq 0$ for all $t$ under any control policy satisfying (\ref{eq:CBF-def}). It therefore suffices to show that $b(x(t)) \geq 0$ for all $t$ implies that $h(x(t)) \geq 0$ for all $t$. If not, then there exists a point satisfying $h(x) = 0$ and $b(x) \geq 0$. This contradicts (\ref{eq:CBF-verification-2}) by Theorem \ref{theorem:Psatz}.
\end{proof}

The conditions of Theorem \ref{theorem:CBF-verification} are convex in the coefficients of $\eta(x)$, $\alpha_{0}(x)$, $\alpha_{1}(x)$, and $\theta_{1}(x),\ldots,\theta_{m}(x)$. Hence there is an exact SOS optimization formulation for verification of a CBF.

One potential drawback of CBF-based control policies is that there may not exist a \emph{smooth} controller satisfying the conditions of the CBF. The following result builds on Theorem \ref{theorem:CBF-verification} to gives sufficient conditions for existence of a smooth safe policy.

\begin{proposition}
\label{prop:smooth-safety}
Suppose that there exist polynomials $\eta(x)$, $\theta_{1}(x),\ldots,\theta_{m}(x)$, SOS polynomials $\alpha_{0}(x)$ and $\alpha_{1}(x)$, and an integer $r$ such that (\ref{eq:CBF-verification-1}) holds. If $\alpha_{1}(x) > 0$ for all $x$, then there exists a smooth safe control policy.
\end{proposition}

\begin{proof}
Consider the control policy defined by $\mu_{i}(x) = -\frac{\theta_{i}(x)}{\alpha_{1}(x)}$. Since $\alpha_{1}(x) > 0$, $\mu_{i}(x)$ is smooth. Eq. (\ref{eq:CBF-verification-1}) implies that
\begin{IEEEeqnarray}{rCl}
\IEEEeqnarraymulticol{3}{l}{
\sum_{i=1}^{m}{(-\theta_{i}(x))\frac{\partial b}{\partial x}g_{i}(x)} + \alpha_{1}(x)\frac{\partial b}{\partial x}f(x)} \\
&=& \eta(x)b(x) + \alpha_{0}(x) + \left(\frac{\partial b}{\partial x} f(x)\right)^{2r} \\
&\geq& \eta(x)b(x)
\end{IEEEeqnarray}
Dividing through by $\alpha_{1}(x)$ gives $$\sum_{i=1}^{m}{\mu_{i}(x)\frac{\partial b}{\partial x}g_{i}(x)} + \frac{\partial b}{\partial x}f(x) \geq \frac{\eta(x)}{\alpha_{1}(x)}b(x).$$ Hence when $b(x) = 0$, we have $\dot{b}(x(t)) \geq 0$, implying that $\{b(x) \geq 0\}$ is positive invariant by Nagumo's Theorem.
\end{proof}

We note that, since $\alpha_{1}(x)$ is SOS, the condition $\alpha_{1}(x) > 0$ can be verified by checking if the matrix representation of $\alpha_{1}(x)$ is positive definite.

\subsection{Verification of Multiple CBFs}
\label{subsec:multi-CBF}
This section considers the problem of checking whether, for a given set of polynomials $b_{1},\ldots,b_{M}$, the set $\bigcap_{i=1}^{M}{\{x: b_{i}(x) \geq 0\}}$ is controlled positive invariant. We have the following equivalent condition for controlled positive invariance.

\begin{proposition}
\label{prop:multi-CBF-conditions}
The set $\bigcap_{i=1}^{M}{\{x : b_{i}(x) \geq 0\}}$ is  controlled positive invariant for some polynomials $b_{1},\ldots,b_{M}$ if and only if, for every $S \subseteq \{1,\ldots,M\}$, there does not exist $x$ satisfying the following properties: (i) $b_{i}(x) = 0$ for all $i \in S$, (ii) $b_{i}(x) \geq 0$ for all $i \notin S$, (iii) for any $u$, there exists $i \in S$ such that 
\begin{equation}
\label{eq:multi-CBF-condition}
\frac{\partial b_{i}}{\partial x}(f(x) + g(x)u) < 0
\end{equation}
\end{proposition}

\begin{proof}
Suppose that, for some $S \subseteq \{1,\ldots,M\}$, there exists $x$ satisfying (i)-(iii), and that $x(0) = x$. Then for any choice of $u(0)$, condition (iii) implies that there exists $i \in S$ such that $b_{i}(x + \delta) < 0$ for some $\delta > 0$. Hence $\bigcap_{i=1}^{M}{\{x : b_{i}(x) \geq 0\}}$ is not controlled positive invariant.

Suppose that, for every $S \subseteq \{1,\ldots,M\}$, there does not exist $x$ satisfying (i)-(iii), and yet the set is not CPI. Let $\mu$ be a control policy that chooses  $u(t)$ satisfying
\begin{equation}
\label{eq:multi-CBF-condition-proof}
\frac{\partial b_{i}}{\partial x}(f(x(t)) + g(x(t))u(t)) \geq 0
\end{equation}
for all $i$ with $b_{i}(x(t)) =0$ at each time $t$ if such a $u$ exists. By (i) and (iii), such a $u$ always exists. Hence $\dot{b}_{i}(x(t)) \geq 0$ whenever $b_{i}(x(t)) = 0$ and positive invariance holds by Nagumo's Theorem.
% Consider a state trajectory $x(t)$ such that $x(0) \in \bigcap_{i=1}^{M}{\{x: b_{i}(x) \geq 0\}}$ and $x(t) \notin \bigcap_{i=1}^{M}{\{x: b_{i}(x) \geq 0\}}$ for some $t \geq 0$. For each $i$, let $t_{i} = \inf{\{t: b_{i}(x(t)) < 0\}}$ and $t^{\ast} = \min{\{t_{i}: i=1,\ldots,M\}}$. By construction, there is a nonempty set $S$ such that $b_{i}(x(t^{\ast})) =0$ for all $i \in S$ and $b_{i}(x(t^{\ast})) \geq 0$ for $i \notin S$. Since $x(t^{\ast})$ satisfies (i) and (ii), there must exist $u$ such that (\ref{eq:multi-CBF-condition-proof}) holds for all $i \in S$, and this $u$ is chosen by the control policy $\mu$. Hence $\dot{b}_{i}(x(t^{\ast})) \geq 0$ for all $i$, creating a contradiction.
\end{proof}

The following intermediate result will be used to construct a convex formulation that is equivalent to the conditions of Proposition \ref{prop:multi-CBF-conditions}. As a preliminary, for any $S=\{i_{1},\ldots,i_{p}\} \subseteq \{1,\ldots,M\}$, define $$\frac{\partial b_{S}}{\partial x} = \left(
\begin{array}{c}
\frac{\partial b_{i_{1}}}{\partial x} \\
\vdots \\
\frac{\partial b_{i_{p}}}{\partial x}
\end{array}
\right)$$

\begin{lemma}
\label{lemma:multi-CBF-helper}
The conditions of Proposition \ref{prop:multi-CBF-conditions} hold if and only if for any $S \subseteq \{1,\ldots,M\}$ there do not exist $x \in \mathbb{R}^{n}$ and $y \in \mathbb{R}^{|S|}$ with (a) $b_{i}(x) = 0$ for all $i \in S$, (b) $b_{i}(x) \geq 0$ for all $i \notin S$, (c) $y \geq 0$, (d) $\left(\frac{\partial b_{S}}{\partial x}g(x)\right)^{T}y = 0$, and (e) $(\frac{\partial b_{S}}{\partial x}f(x))^{T}y < 0$.
\end{lemma}

\begin{proof}
It suffices to show that conditions (c)-(e) above are equivalent to condition (iii) of Proposition \ref{prop:multi-CBF-conditions}. We have that condition (iii) of Proposition \ref{prop:multi-CBF-conditions} holds if for any $x$ satisfying $b_{i}(x) = 0$ for all $i \in S$ and $b_{i}(x) \geq 0$ for all $i \in S$, there exists $u$ satisfying $$\left(\frac{\partial b_{S}}{\partial x}\right)g(x)u \geq -\frac{\partial b_{S}}{\partial x}f(x).$$ By Farkas's Lemma, this is equivalent to the non-existence of $y$ satisfying conditions (c)-(e).
\end{proof}

Based on this result, we can define the following equivalent conditions for a set of polynomials to define a controlled positive invariant set. 

\begin{theorem}
\label{theorem:multi-CBF-conditions}
For a set of polynomials $b_{1},\ldots,b_{M}$, the set $\bigcap_{i=1}^{M}{\{x : b_{i}(x) \geq 0\}}$ is controlled positive invariant if and only if, for all $S \subseteq \{1,\ldots,M\}$, there exists a polynomial $$\eta_{S} \in \mathcal{I}[(b_{i} : i \in S), \ (\frac{\partial b_{i}}{\partial x}g_{j}y_{i}: i \in S, j=1,\ldots,m)],$$ integers $\{r_{i} : i \in S\}$, and a polynomial $$\lambda_{S} \in \Sigma\left[(-\frac{\partial b_{i}}{\partial x}f(x) : i \in S), (y_{i}: i \in S), (b_{i}: i \notin S)\right]$$ such that 
\begin{equation}
\label{eq:multi-CBF-condition-1}
\eta_{S} 
+ \lambda_{S} + \left(\prod_{i \in S}{\left(\frac{\partial b_{i}}{\partial x}f(x)\right)^{r_{i}}}\right)^{2} = 0
\end{equation}

Moreover, for a given safe region $\mathcal{C} = \bigcap_{i=1}^{M}{\{x : h_{i}(x) \geq 0\}}$, a control policy with CBFs $b_{1},\ldots,b_{N}$ ensures safety if there exist polynomials $\beta_{i} \in \Sigma[b_{1},\ldots,b_{N}]$ and $\omega_{i}$ such that 
\begin{equation}
\label{eq:multi-CBF-condition-2}
\beta + \omega(x)h_{i}(x) + 1 = 0.
\end{equation}
for all $i=1,\ldots,M$
\end{theorem}

\begin{proof}
Eq. (\ref{eq:multi-CBF-condition-1}) is equivalent to the conditions of Lemma \ref{lemma:multi-CBF-helper} by Theorem \ref{theorem:Psatz}. Furthermore, in order for the control policy to ensure safety, we must have that there is no point with $h_{i}(x) = 0$ and $b_{j}(x) \geq 0$ for $j=1,\ldots,M$. This condition is equivalent to (\ref{eq:multi-CBF-condition-2}) by Theorem \ref{theorem:Psatz}.
\end{proof}

While Theorem \ref{theorem:multi-CBF-conditions} leads to a convex formulation for verifying multiple CBFs, it requires solving SOS programs with $2^{M}$ SOS constraints. High-Order CBFs are a tractable subclass of multiple CBF-based control policies; their tractability follows from the fact that the control input $u$ is only used to ensure positive invariance of $\psi_{r}$, while positive invariance of the remaining sets is satisfied by construction. We have the following approach.

\begin{theorem}
\label{theorem:HOCBF-verification}
If $b(x)$ is a polynomial with relative degree $r$ with respect to (\ref{eq:dynamics}), then $b(x)$ and $\psi_{0},\ldots,\psi_{r}$ define a HOCBF if and only if there exist polynomials $\eta(x)$, $\theta_{1}(x),\ldots,\theta(x)$, $\gamma \in \Sigma[L_{f}^{r}b(x) + O(b(x)), \psi_{0},\ldots,\psi_{r}]$, and an integer $s$ such that 
\begin{multline}
\label{eq:HOCBF-verification-1}
\eta(x)\psi_{r}(x) + \sum_{i=1}^{r}{\theta_{i}(x)L_{g}L_{f}^{r-1}b(x)} + \gamma \\
+ (L_{f}^{r}b(x) + O(b(x)))^{2s}
\end{multline}
Moreover, the set $\bigcap_{i=0}^{r}{C_{i}}$ is a subset of $\mathcal{C}$ if and only if there exist $\beta \in \Sigma[\psi_{0},\ldots,\psi_{r}]$ and a polynomial $w(x)$ such that 
\begin{equation}
\label{eq:HOCBF-verification-2}
\beta + w(x)h(x) + 1 = 0
\end{equation}
\end{theorem}

\begin{proof}
By Theorem \ref{theorem:HOCBF-safety}, $\{b(x) \geq 0\}$ is controlled positive invariant if (\ref{eq:HOCBF-def}) holds for some $u$ at each $x \in \bigcap_{i=0}^{r}{C_{i}}$. Such a $u$ exists iff there is no $x$ with $\psi_{i}(x) \geq 0$ for $i=0,\ldots,r$, $\psi_{r}(x) = 0$, $L_{f}^{r-1}L_{g}b = 0$, and $L_{f}^{r}b + O(b(x)) < 0$. This is equivalent to (\ref{eq:HOCBF-verification-1}) by Theorem \ref{theorem:Psatz}.

Now, we want to show that if $x(t) \in C_{i}$ for $i=0,\ldots,r$ and $h(x(0)) \geq 0$, then $h(x(t)) \geq 0$ for all $t$ if (\ref{eq:HOCBF-verification-2}) holds. If (\ref{eq:HOCBF-verification-2}) holds, then there is no $x$ satisfying $x \in C_{i}$ for $i=0,\ldots,r$ and $h(x) = 0$. Since $x(t) \in C_{i}$ for all $t$ and $i=0,\ldots,r$, this implies that $x(t)$ never reaches the boundary of $\mathcal{C}$ and hence remains in $\mathcal{C}$ for all time $t$.
\end{proof}

\subsection{Verification of Semi-Algebraic Sets}
\label{subsec:semialgebraic}
A set $\mathcal{S}$ is semi-algebraic if there exist polynomials $b_{ij}: i=1,\ldots,N, j=1,\ldots,K$ for some integers $N$ and $K$ such that 
\begin{equation}
\label{eq:semi-algebraic}
\mathcal{S} = \bigcup_{i=1}^{N}{\bigcap_{j=1}^{K}{\{x: b_{ij}(x) \geq 0\}}}.
\end{equation}
In what follows, we present an approach for verifying controlled positive invariance of semi-algebraic sets. As a preliminary, we consider the case where 
\begin{equation}
\label{eq:union}
\mathcal{S} = \bigcup_{i=1}^{N}{\{x:b_{i}(x) \geq 0\}}.
\end{equation}
for polynomials $b_{1},\ldots,b_{N}$.

\begin{lemma}
\label{lemma:union-CPI}
The set $\mathcal{S}$ defined in (\ref{eq:union}) is controlled positive invariant if and only if for any $S \subseteq \{1,\ldots,N\}$, there does not exist $x$ with $b_{i}(x) = 0$ for $i \in S$, $b_{i}(x) < 0$ for $i \notin S$, $\frac{\partial b_{i}}{\partial x}g(x) = 0$ for $i \in S$, and $\frac{\partial b_{i}}{\partial x}f(x) < 0$ for $i \in S$. 
\end{lemma}

\begin{proof}
Suppose that there exists such an $x$. We have that $x$ lies outside the sets $\{b_{i}(x) \geq 0\}$ for $i \notin S$ and at the boundary of the sets $\{b_{i}(x) \geq 0\}$ for $i \in S$. Furthermore, for all $i \in S$, we have $\dot{b}_{i}(x) < 0$ regardless of the control input. Hence the state trajectory will leave the set $\mathcal{S}$ if $x(0) = x$.

%Conversely, suppose that $\mathcal{S}$ is not CPI. Let $x(0)$

Conversely, let $\mu$ be a control policy such that, for all sets $S$ and all $x$ satisfying $b_{i}(x) = 0$ for $i \in S$ and $b_{i}(x) < 0$ for $i \notin S$, $$\frac{\partial b_{i}}{\partial x}(f(x) + g(x)\mu(x)) \geq 0.$$ Hence for any $x$ on the boundary of $\mathcal{S}$, there exists at least one $i$ with $b_{i}(x) = 0$ and $\dot{b}_{i}(x) \geq 0$. We then have that, if $x(t)$ reaches the boundary of $\mathcal{S}$, then there exists $\delta > 0$ such that $x(t^{\prime}) \in \mathcal{S}$ for $t^{\prime} \in (t,t+\delta)$.
\end{proof}

The conditions of Lemma \ref{lemma:union-CPI} can be mapped to an SOS program via the following.

\begin{theorem}
    \label{theorem:union-SOS}
    The set $\mathcal{S}$ defined in (\ref{eq:union}) is CPI if and only if for any $S \subseteq \{1,\ldots,N\}$, there exists $$\eta_{S} \in \mathcal{I}[(b_{i} : i \in S), \left(\frac{\partial b_{i}}{\partial x}g_{j}(x) : i\in S, j=1,\ldots,m\right)]$$ and $$\lambda_{S} \in \Sigma[(-b_{i}(x) : i \notin S), (-\frac{\partial b_{i}}{\partial x}f(x) : i \in S)],$$ and integers $r_{i}^{S}$ for $i=1,\ldots,N$ such that
    \begin{equation}
    \label{eq:union-SOS}
    \eta_{S} + \lambda_{S} + \prod_{i \in S}\left(\frac{\partial b_{i}}{\partial x}f(x)\right)^{2r_{i}^{S}}\prod_{i \notin S}{\left(b_{i}(x)\right)^{2r_{i}^{S}}} = 0.
    \end{equation}
    Moreover, the set $\mathcal{S}$ is contained in the safe region if, for all $i =1,\ldots,N$, there exist SOS polynomials $\beta_{i1}$ and $\beta_{i0}$ as well as a polynomial $\omega_{i}$ such that 
    \begin{equation}
    \label{eq:union-containment}
    \beta_{i1}b_{i} + \omega_{i}h + \beta_{i0} + 1 = 0.
    \end{equation}
\end{theorem}

\begin{proof}
Eq. (\ref{eq:union-SOS}) is equivalent to the conditions of Lemma \ref{lemma:union-CPI} by Theorem \ref{theorem:Psatz}. The remainder of the proof follows by applying Eq. (\ref{eq:CBF-verification-2}) to each function $b_{1},\ldots,b_{N}$.
\end{proof}

We next consider semi-algebraic sets of the form (\ref{eq:semi-algebraic}). We have the following result on controlled positive invariance of such sets.

\begin{lemma}
\label{lemma:semi-algebraic-CPI}
A semi-algebraic set (\ref{eq:semi-algebraic}) is CPI if and only if for all $S \subseteq \{1,\ldots,N\}$, subsets $T_{i} \subseteq \{1,\ldots,K\}$ for $i \in S$, and indices $j_{i} \in \{1,\ldots,K\}$ for $i \notin S$, there does not exist $x$ satisfying (a) $b_{ij}(x) = 0$ for $i \in S$, $j \in T_{i}$ (b) $b_{ij}(x) > 0$ for $i \in S$, $j \notin T_{i}$, (c) $b_{ij_{i}}(x) < 0$ for $i \notin S$, and (d) for all $u \in \mathbb{R}^{m}$ and $i \in S$, $$\frac{\partial b_{ij}}{\partial x}(f(x) + g(x)u) < 0$$ for some $j \in T_{i}$.
\end{lemma}

The proof generalizes the proofs of Proposition \ref{prop:multi-CBF-conditions} and Lemma \ref{lemma:union-CPI} and is omitted due to space constraints.

We now formulate equivalent conditions to Lemma \ref{lemma:semi-algebraic-CPI} that can be mapped to an SOS program.

\begin{lemma}
\label{lemma:semi-algebraic-Farkas}
A semi-algebraic set (\ref{eq:semi-algebraic}) is CPI if and only if for all $S \subseteq \{1,\ldots,N\}$, subsets $T_{i} \subseteq \{1,\ldots,K\}$ for $i \in S$, and indices $j_{i} \in \{1,\ldots,K\}$ for $i \notin S$, there do not exist $x \in \mathbb{R}^{n}$ and $\{y_{i} : i \in S\}$ such that (i) $b_{ij}(x) = 0$ for $i \in S$, $j \in T_{i}$ (ii) $b_{ij}(x) > 0$ for $i \in S$, $j \notin T_{i}$, (iii) $b_{ij_{i}}(x) < 0$ for $i \notin S$, (iv) $y_{i} \geq 0$ for all $i \in S$, (v) $\left(\frac{\partial b_{T_{i}}}{\partial x}g(x)\right)^{T}y = 0$, and (vi) $\left(\frac{\partial b_{T_{i}}}{\partial x}f(x)\right)^{T}y < 0$, where $b_{T_{i}}$ is defined as in Lemma \ref{lemma:semi-algebraic-CPI}.
\end{lemma}

\begin{proof}
Conditions (i)-(iii) follow directly from conditions (a)-(c) of Lemma \ref{lemma:semi-algebraic-CPI}. Conditions (iv) and (iv) are equivalent to condition (d) by Farkas's Lemma.
\end{proof}

We finally give a convex framework for verifying positive invariance of semialgebraic sets.
\begin{theorem}
\label{theorem:Psatz-semialgebraic}
A semi-algebraic set (\ref{eq:semi-algebraic}) is CPI if and only if for all $S \subseteq \{1,\ldots,N\}$, subsets $T_{i} \subseteq \{1,\ldots,K\}$ for $i \in S$, and indices $j_{i} \in \{1,\ldots,K\}$ for $i \notin S$, there exist polynomials 
\begin{displaymath}
\eta \in \mathcal{I}\left[(b_{ij} : i \in S, j \in T_{i}), \left(\frac{\partial b_{T_{i}}}{\partial x}\right)^{T}y\right] 
\end{displaymath}
and 
\begin{multline*}
\lambda \in \Sigma\left[(b_{ij} : i \in S, j \notin T_{i}),(y_{i}: i \in S), (-b_{ij_{i}} : i \notin S), \right. \\
\left.-\left(\frac{\partial b_{T_{i}}}{\partial x}f(x)\right)^{T}y\right]
\end{multline*}
along with nonnegative integers $\{r_{ij} : i \in S, j \notin T_{i}\}$, $\{s^{i} : i \notin S\}$ and $v$ such that $$\eta + \lambda + \left[\left(\prod_{\stackrel{i \in S}{j \notin T_{i}}}{b_{ij}^{r_{ij}}}\right)\left(\prod_{i \notin S}{(b_{ij_{i}})^{s_{i}}}\right) \left(\left(\frac{\partial b_{T_{i}}}{\partial x}f(x)\right)^{T}y\right)^{v}\right]^{2} = 0.$$
\end{theorem}

\begin{proof}
The result follows from Lemma \ref{lemma:semi-algebraic-CPI} and Theorem \ref{theorem:Psatz}.
\end{proof}

\subsection{Dynamics with Trigonometric Functions}
\label{subsec:trig}
In what follows, we present an approach for verifying safety of systems with dynamics that contain trigonometric functions. We consider a system (\ref{eq:dynamics}) such that there exists $l \in \{1,\ldots,n\}$ and polynomials $\overline{f}$, $\overline{g}$, and $\overline{b}$ such that
\begin{IEEEeqnarray}{rCl}
\label{eq:trig-dynamics-1}
f(x) &=& \overline{f}(x_{1},\ldots,x_{l},r_{1},\ldots,r_{L}) \\
\label{eq:trig-dynamics-2}
g(x) &=& \overline{g}(x_{1},\ldots,x_{l},r_{1},\ldots,r_{L}) \\
\label{eq:trig-dynamics-3}
b(x) &=& \overline{b}(x_{1},\ldots,x_{l},r_{1},\ldots,r_{L})\\
\label{eq:trig-dynamics-4}
h_{m}(x) &=& \overline{h}_{m}(x_{1},\ldots,x_{l},r_{1},\ldots,r_{L})
\end{IEEEeqnarray}
where $r_{i} = \phi(x_{j})$ for some $j \in \{(l+1),\ldots,n\}$ and $\phi \in \{\sin, \cos, \tan, \csc, \sec, \cot\}$. This condition implies that there exist a subset of variables $x_{l+1},\ldots,x_{n}$ that only appear as arguments of trigonometric functions. We further assume that each of (\ref{eq:trig-dynamics-1})--(\ref{eq:trig-dynamics-4}) is well-defined within the safe region, i.e., if $\tan{x_{i}}$ appears in the system dynamics, then $\cos{x_{i}} \neq 0$ throughout the safe region.

For each $i \in \{(l+1),\ldots,n\}$, we define auxiliary variables $z_{ij}$, $j=1,\ldots,6$. Each variable will define a different trigonometric function of $x_{i}$, i.e., $z_{i1} = \sin{x_{i}}$, $z_{i2} = \cos{x_{i}}$, $z_{i3} = \tan{x_{i}}$, $z_{i4} = \csc{x_{i}}$, $z_{i5} = \sec{x_{i}}$, and $z_{i6} = \cot{x_{i}}$. We note that not all auxiliary variables may be required to describe the system dynamics, for example, only $z_{i1}$ and $z_{i2}$ are required if the system dynamics only contain functions of $\sin{x_{i}}$ and $\cos{x_{i}}$.

These auxiliary variables are incorporated into the Lie derivative computations of $b(x)$ as follows. For $i \leq l$, we have $\frac{\partial b}{\partial x_{i}} = \frac{\partial \overline{b}}{\partial x_{i}}$. For $i \in \{(l+1),\ldots,n\}$, we have $$\frac{\partial b}{\partial x_{i}} = \sum_{\stackrel{j: z_{ij} = r_{k}}{k\in\{1,\ldots,L\}}}{\frac{\partial \overline{b}}{\partial r_{k}}z_{ij}^{\prime}},$$ where 
\begin{displaymath}
z_{ij}^{\prime} = \left\{
\begin{array}{llll}
z_{i2}, & j=1 & -z_{i4}z_{i6}, & j =4 \\
-z_{i1}, & j=2 & z_{i3}z_{i5}, & j=5 \\
z_{i5}^{2}, & j=3 & -z_{i4}^{2}, & j=6
\end{array}
\right.
\end{displaymath}

Finally, to ensure that the variables $z_{ij}$ are consistent with trigonometric functions, we impose the constraints
\begin{IEEEeqnarray*}{rCl}
z_{i1}^{2} + z_{i2}^{2} &=& 1, \quad -1 \leq z_{i1} \leq 1, \quad -1 \leq z_{i2} \leq 1 \\
z_{i2}z_{i3} &=& z_{i1}, \quad z_{i1}z_{i4} = 1, \quad z_{i2}z_{i5} = 1, \quad z_{i3}z_{i6} = 1
\end{IEEEeqnarray*}

We define polynomials $\lambda_{i} = z_{i1}^{2} + z_{i2}^{2} - 1$, $\kappa_{ij} = z_{ij}+1$, $\zeta_{ij} = 1-z_{ij}$, $\chi_{i1} = z_{i1}-z_{i2}z_{i3}$, $\chi_{i2} = z_{i1}z_{i4}-1$, $\chi_{i3} = z_{i2}z_{i5}-1$, and $\chi_{i4} = z_{i3}z_{i6}-1$. We have the following result.

\begin{proposition}
\label{prop:trig-conditions}
For a system described by (\ref{eq:dynamics}) and (\ref{eq:trig-dynamics-1})--(\ref{eq:trig-dynamics-3}), suppose there do not exist $x_{1},\ldots,x_{l}$ and $z_{ij}$, $i=(l+1),\ldots,n$, $j=1,\ldots,6$ satisfying $b(x,z) = 0$, $\frac{\partial b}{\partial x}g(x,z) = 0$, $\frac{\partial b}{\partial x}f(x) < 0$, $\lambda_{i}(x,z) = 0$,$i=(l+1),\ldots,n$, $\kappa_{ij}(x,z) \geq 0$, $\zeta_{ij} \geq 0$ for $i=(l+1),\ldots,n$, $j=1,2$, and $\chi_{ij}(x,z) = 0$ for $i=(l+1),\ldots,n$, $j=1,\ldots,4$. Then the set $\{b(x) \geq 0\}$ is controlled positive invariant.
\end{proposition}

\begin{proof} 
Suppose that $\{b(x) \geq 0\}$ is not controlled positive invariant. Then there exists $x^{\prime}$ such that $b(x^{\prime}) = 0$ and $\dot{b}(x^{\prime}) < 0$ for any $u$. For this to be true, we must have $\frac{\partial b}{\partial x}g(x^{\prime}) = 0$ and $\frac{\partial b}{\partial x}f(x^{\prime}) < 0$. We can then choose $x_{1},\ldots,x_{l}$ and $z_{ij}$ by $x_{i} = x_{i}^{\prime}$ for $i \in \{1,\ldots,l\}$ and $z_{ij} = \phi(x_{i})$ for $i=(l+1),\ldots,n$, $j=1,\ldots,6$, where $\phi$ denotes the appropriate trigonometric function. 
\end{proof}

This construction then leads to a SOS formulation for verifying a CBF with trigonometric dynamics.

\begin{theorem}
\label{theorem:trig-verification}
Suppose that there exist polynomials 
\begin{multline*}
\eta \in \mathcal{I}[b,(\frac{\partial b}{\partial x}g_{i} : i=1,\ldots,m), \\
(\lambda_{i} : i=(l+1),\ldots,n), (\chi_{ij} = i=(l+1),\ldots,n, j=1,\ldots,4)]
\end{multline*}
and 
\begin{multline*}
\beta \in \Sigma\left[-\frac{\partial b}{\partial x}f(x), (\kappa_{ij}: i=(l+1),\ldots,n, j=1,2), \right.\\
\left.(\zeta_{ij}: i =(l+1),\ldots,n, j=1,2)\right]
\end{multline*}
such that  
\begin{displaymath}
\eta 
+ \beta + \left(\frac{\partial b}{\partial x}f(x)\right)^{2r} = 0.
\end{displaymath}
Then $\{b(x) \geq 0\}$ is controlled positive invariant. Moreover, if there exist 
\begin{multline*}
\tau \in \mathcal{I}\left[h, (\rho_{i}:i=(l+1),\ldots,n),\right. \\
\left.(\chi_{ij}:i=(l+1),\ldots,n,j=1,\ldots,4)\right]
\end{multline*}
and 
\begin{multline*}
\phi \in \Sigma\left[b(x),(\kappa_{ij}:i=(l+1),\ldots,n,j=1,2), \right. \\
\left.(\zeta_{ij}: i=(l+1),\ldots,n, j=1,2)\right]
\end{multline*}
such that $$\tau + \phi + 1 = 0,$$
then the condition $\{h(x) \geq 0\}$ is satisfied for all time $t$.
\end{theorem}

\begin{proof}
Proposition \ref{prop:trig-conditions} gives sufficient conditions for safety based on non-existence of solutions to a system of polynomial equations.
\end{proof}

Theorem \ref{theorem:trig-verification} gives an SOS program for verifying safety of CBFs with trigonometric functions, at the cost of introducing additional polynomial constraints and variables.

\subsection{Actuation Constraints}
\label{subsec:verification-actuation}
We next consider systems with actuation constraints of the form $Au \leq c$ for some matrix $A \in \mathbb{R}^{p \times m}$ and $c \in \mathbb{R}^{p}$. The following result gives a necessary and sufficient condition for $b(x)$ to be a CBF in the presence of such an actuation constraint.

\begin{proposition}
\label{prop:actuation-condition}
The function $b(x)$ is a CBF if and only if there do not exist $x \in \mathbb{R}^{n}$ and $y \in \mathbb{R}^{p+1}$ satisfying
\begin{multline}
\label{eq:actuation-condition}
b(x) = 0, \ \left(
\begin{array}{c}
-\frac{\partial b}{\partial x}g(x) \\
A
\end{array}
\right)^{T}y = 0, \\ \left(
\begin{array}{c}
\frac{\partial b}{\partial x}f(x) \\
c
\end{array}
\right)^{T}y < 0, \ y \geq 0
\end{multline}
\end{proposition}

\begin{proof}
In order to ensure that $\dot{b}(x(t)) \geq 0$ whenever $b(x(t)) = 0$, it is necessary and sufficient to ensure that for every $x$ with $b(x) = 0$, there exists $u$ satisfying
\begin{IEEEeqnarray*}{rCl}
-\frac{\partial b}{\partial x}g(x)u &\leq& \frac{\partial b}{\partial x}f(x) \\
Au &\leq& c
\end{IEEEeqnarray*}
By Farkas's Lemma, the existence of such a $u$ is equivalent to the non-existence of $y$ satisfying (\ref{eq:actuation-condition}).
\end{proof}

Define a set of polynomials $d_{1},\ldots,d_{m}$ by $$d_{i} = \left(-\frac{\partial b}{\partial x}g_{i}(x)\right)y_{1} + \sum_{j=1}^{p}{A_{ji}y_{j+1}},$$ so that the condition $$\left(
\begin{array}{c}
-\frac{\partial b}{\partial x}g(x) \\
A
\end{array}
\right)^{T}y = 0$$ is equivalent to $d_{i} = 0$ for $i=1,\ldots,m$. We now give equivalent SOS conditions for CBFs with actuation constraints. 

\begin{theorem}
\label{theorem:Psatz-actuation}
The function $b(x)$ is a CBF under the actuation constraint $Au \leq b$ if and only if there exists a polynomial $$\eta \in \mathcal{I}\left[b,(d_{i}: i=1,\ldots,m)\right],$$ a polynomial $$\beta \in \Sigma\left[y_{1},\ldots,y_{p+1}, -\left(
\begin{array}{c}
\frac{\partial b}{\partial x}f(x)\\
c
\end{array}
\right)^{T}y\right],$$ and integer $r$ with
\begin{displaymath}
\eta
+ \beta + \left[\left(\begin{array}{c}
\frac{\partial b}{\partial x}f(x) \\
c
\end{array}
\right)^{T}y\right]^{2r} = 0
\end{displaymath}
\end{theorem}

\begin{proof}
The proof follows from applying Theorem \ref{theorem:Psatz} to the polynomial constraints (\ref{eq:actuation-condition}) in Proposition \ref{prop:actuation-condition}.
\end{proof}

We observe that this approach can be applied to incorporating multiple safety constraints $h_{1},\ldots,h_{M}$ as well as verifying multiple CBFs as in Section \ref{subsec:multi-CBF}. We omit this generalization due to space constraints and for simplicity of the exposition.


\subsection{Euler-Lagrange Dynamics}
\label{subsec:Lagrangian}
In what follows, we consider a generalization of (\ref{eq:dynamics}) to systems with Euler-Lagrange dynamics that are described by  ODEs of the form
\begin{equation}
\label{eq:Lagrangian-dynamics}
\Phi_{1}(x,\dot{x}) + \Phi_{2}(x,\dot{x})\ddot{x} = u
\end{equation}
We further assume that the control input is constrained by $u(t) \in \mathcal{U} = [u_{min}^{1},u_{max}^{1}] \times \cdots \times [u_{min}^{m},u_{max}^{m}]$. The goal is to verify a CBF of the form $b(x,\dot{x})$. We have the following initial result.

\begin{proposition}
\label{prop:Lagrangian-Nagumo}
The set $\{(x,\dot{x}): b(x,\dot{x}) \geq 0\}$ is controlled positive invariant if, for any $(x,\dot{x})$ with $b(x,\dot{x}) = 0$, there exists $u$ such that 
\begin{equation}
\label{eq:Lagrangian-CPI}
\frac{\partial b}{\partial x}\dot{x} + \frac{\partial b}{\partial \dot{x}}\ddot{x} \geq 0
\end{equation}
for any $\ddot{x}$ satisfying (\ref{eq:Lagrangian-dynamics}).
\end{proposition}

\begin{proof}
By Nagumo's Theorem, the set is controlled positive invariant if and only if, for any $(x,\dot{x})$ with $b(x,\dot{x}) = 0$, we have $\dot{b}(x,\dot{x}) \geq 0$. This is equivalent to the existence of $u$ that ensures (\ref{eq:Lagrangian-CPI}) for all feasible values of $\ddot{x}$, i.e., for all solutions to (\ref{eq:Lagrangian-dynamics}).
\end{proof}

We will next derive conditions for verifying the conditions of Proposition \ref{prop:Lagrangian-Nagumo} for a given function $b$. As a preliminary, we have the following generalization of Farkas's Lemma to strict inequalities.

\begin{lemma}[\cite{dinh2014farkas}]
\label{lemma:generalized-Farkas}
Exactly one of the following statements is true:
\begin{enumerate}
\item There exists an $x$ satisfying $Ax < b$ and $Bx \leq c$.
\item There exist $y$ and $z$ that satisfy $y\geq 0$, $z \geq 0$, $A^{T}y + B^{T}z = 0$, and either $b^{T}y + c^{T}z < 0$ or ($b^{T}y + c^{T}z = 0$ and $y \neq 0$).
\end{enumerate}
\end{lemma}

We note two special cases of this lemma. First, if we are given an equality constraint $Bx = c$ instead of an inequality constraint, then we can remove the constraint $z \geq 0$. Second, if $b=0$ and $c=0$, then the second condition of Lemma \ref{lemma:generalized-Farkas} reduces to $y \geq 0$, $z \geq 0$, $A^{T}y + B^{T}z = 0$, and $y \neq 0$.

We next present a preliminary result before giving our main conditions.

\begin{lemma}
\label{lemma:Lagrange-inner-Farkas}
The function $b(x,\dot{x})$ is a CBF for (\ref{eq:Lagrangian-dynamics}) if and only if, for every $(x,\dot{x})$ with $b(x,\dot{x}) = 0$, at least one of the following conditions holds:
\begin{enumerate}
\item There exists $y \in \mathbb{R}$, $z \in \mathbb{R}^{m}$, and a vertex $s$ of the hypercube $\mathcal{U}$ such that $y \geq 0$ and 
\begin{IEEEeqnarray}{rCl}
\label{eq:Inner-Farkas-1}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T}y + \Phi_{2}(x,\dot{x})^{T}z &=& 0 \\
\label{eq:Inner-Farkas-2}
-\left(\frac{\partial b}{\partial x}\dot{x}\right)y - \Phi_{1}(x,\dot{x})^{T}z + s^{T}z &<& 0 
\end{IEEEeqnarray}
\item There exist $z \in \mathbb{R}^{m}$, $y \in \mathbb{R}$, and vertices $s,s^{\prime}$ of the hypercube $\mathcal{U}$  such that $y > 0$ and
\begin{IEEEeqnarray}{rCl}
\label{eq:Inner-Farkas-3}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T}y + \Phi_{2}(x,\dot{x})^{T}z &=& 0 \\
\label{eq:Inner-Farkas-4}
-\left(\frac{\partial b}{\partial x}\dot{x}\right)y - \Phi_{1}(x,\dot{x})^{T}z +s^{T}z &\leq& 0 \\
\label{eq:Inner-Farkas-5}
-\left(\frac{\partial b}{\partial x}\dot{x}\right)y - \Phi_{1}(x,\dot{x})^{T}z +(s^{\prime})^{T}z &\geq& 0 
\end{IEEEeqnarray}
\end{enumerate}
\end{lemma}

\begin{proof}
The conditions of Proposition \ref{prop:Lagrangian-Nagumo} can be stated as, for some $u \in \mathcal{U}$, there does not exist $\ddot{x}$ satisfying (\ref{eq:Lagrangian-dynamics}) and (\ref{eq:Lagrangian-CPI}). By Lemma \ref{lemma:generalized-Farkas}, these conditions are equivalent to at least one of the following  holding:
\begin{enumerate}
\item[(i)] There exists $u \in \mathcal{U}$, $y \in \mathbb{R}_{\geq 0}$, and $z \in \mathbb{R}^{m}$ such that
\begin{IEEEeqnarray}{rCl}
\label{eq:inner-Farkas-intermediate-1}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T}y + \Phi_{2}(x,\dot{x})^{T}z &=& 0 \\
\label{eq:inner-Farkas-intermediate-2}
-\left(\frac{\partial b}{\partial x}\dot{x}\right)y + (-\Phi_{1}(x,\dot{x}) + u)^{T}z &<& 0
\end{IEEEeqnarray}
\item[(ii)] There exists $u \in \mathcal{U}$, $y \in \mathbb{R}_{> 0}$, and $z \in \mathbb{R}^{m}$ such that 
\begin{IEEEeqnarray*}{rCl}
\label{eq:inner-Farkas-intermediate-3}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T}y + \Phi_{2}(x,\dot{x})^{T}z &=& 0 \\
\label{eq:inner-Farkas-intermediate-4}
-\left(\frac{\partial b}{\partial x}\dot{x}\right)y + (-\Phi_{1}(x,\dot{x}) + u)^{T}z &=& 0
\end{IEEEeqnarray*}
\end{enumerate}
Turning first to condition (i), we have that $u^{T}z$ is minimized at the vertices of $\mathcal{U}$. Hence, it is sufficient to check whether (\ref{eq:inner-Farkas-intermediate-1}) and (\ref{eq:inner-Farkas-intermediate-2}) hold at the vertices, resulting in condition 1 of the lemma.

Next, we examine condition (ii). For a given value of $z$, let $v_{min}$ and $v_{max}$ be the minimum and maximum of $u^{T}z$ over $u \in \mathcal{U}$, respectively.  Eq. (\ref{eq:inner-Farkas-intermediate-4}) holds iff 
\begin{multline*}
-\left(\frac{\partial b}{\partial x}\dot{x}\right)y + (-\Phi_{1}(x,\dot{x}))^{T}z + v_{min} \leq 0 \\ 
\leq -\left(\frac{\partial b}{\partial x}\dot{x}\right)y + (-\Phi_{1}(x,\dot{x}))^{T}z + v_{max}.
\end{multline*}
Since $v_{min}$ and $v_{max}$ are achieved at vertices of $\mathcal{U}$, this is equivalent to condition 2 of the lemma.
\end{proof}

As a corollary to Lemma \ref{lemma:Lagrange-inner-Farkas}, a safe control policy can be constructed for a system (\ref{eq:Lagrangian-dynamics}) by selecting $u \in \mathcal{U}$, $y > 0$, and $z \in \mathbb{R}^{m}$ such that 
\begin{IEEEeqnarray*}{rCl}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T}y + \Phi_{2}(x,\dot{x})^{T}z &=& 0 \\
-\left(\frac{\partial b}{\partial \dot{x}}\dot{x}\right)y + (-\Phi_{1}(x,\dot{x}) + u)^{T}z &\leq& 0
\end{IEEEeqnarray*}

We now present a further equivalent condition for $b(x,\dot{x})$ to be a CBF. As a preliminary, for vertices $s,s^{\prime}$ of $\mathcal{U}$, define
\begin{IEEEeqnarray*}{rCl}
A(s,x,\dot{x}) &=& (-\frac{\partial b}{\partial x}\dot{x} \ (s-\Phi_{1}(x,\dot{x}))^{T}) \\
B(x,\dot{x}) &=& \left(
\begin{array}{cc}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T} & \Phi_{2}(x,\dot{x})^{T} \\
-\left(\frac{\partial b}{\partial \dot{x}}\right)^{T} & -\Phi_{2}(x,\dot{x})^{T} \\
-I & 0 
\end{array}
\right) \\
C &=& (-I \ 0) \\
D(s,s^{\prime},x,\dot{x}) &=& \left(
\begin{array}{cc}
\left(\frac{\partial b}{\partial \dot{x}}\right)^{T} & \Phi_{2}(x,\dot{x})^{T} \\
-\left(\frac{\partial b}{\partial \dot{x}}\right)^{T} & -\Phi_{2}(x,\dot{x})^{T} \\
-\left(\frac{\partial b}{\partial x}\dot{x}\right) & (-\Phi_{1}(x,\dot{x})^{T} + s^{T}) \\
\frac{\partial b}{\partial x}\dot{x} & (\Phi_{1}(x,\dot{x}) - (s^{\prime})^{T})
\end{array}
\right)
\end{IEEEeqnarray*}

\begin{lemma}
\label{lemma:Lagrangian-outer-Farkas}
The function $b$ is a CBF for the system with dynamics (\ref{eq:Lagrangian-dynamics}) if and only if there do not exist $x$, $\dot{x}$, $w_{s} \geq 0$, $v_{s,s^{\prime}} \geq 0$, $r_{s} \geq 0$, and $q_{s,s^{\prime}} \geq 0$ with $w_{s},v_{s,s^{\prime}} \neq 0$ where $s$ and $s^{\prime}$ are indexed as the vertices in $\mathcal{U}$ such that $A_{s}^{T}w_{s} + B^{T}r_{s} = 0$ for all $s$ vertices of $\mathcal{U}$ and $C^{T}v_{s,s^{\prime}} + D(s,s^{\prime},x,\dot{x})^{T}q_{s,s^{\prime}} = 0$ for all $s,s^{\prime}$ vertices of $\mathcal{U}$, and $b(x,\dot{x}) = 0$.
\end{lemma}

\begin{proof}
By Lemma \ref{lemma:Lagrange-inner-Farkas}, $b(x,\dot{x})$ is a CBF if and only if for every $x,\dot{x}$ with $b(x,\dot{x}) = 0$, there exist $y \geq 0$, $z \in \mathbb{R}^{m}$, and a vertex $s$ such that (\ref{eq:Inner-Farkas-1}) and (\ref{eq:Inner-Farkas-2}) hold, or there exist $z \in \mathbb{R}^{m}$, $y > 0$, and vertices $s,s^{\prime}$ such that (\ref{eq:Inner-Farkas-3})--(\ref{eq:Inner-Farkas-5}) hold. Equivalently, $b$ is a CBF if and only if there do not exist $x,\dot{x}$ with $b(x,\dot{x}) = 0$ such that conditions (\ref{eq:Inner-Farkas-1}) and (\ref{eq:Inner-Farkas-2}) fail to hold for all $y \geq 0$, $z \in \mathbb{R}^{m}$, and $s$ and the conditions (\ref{eq:Inner-Farkas-3})--(\ref{eq:Inner-Farkas-5}) fail to hold for all $y > 0$, $z \in \mathbb{R}^{m}$, and vertices $s,s^{\prime}$. 

By Farkas's Lemma, the former condition is equivalent to $A(s,x,\dot{x})^{T}w_{s} + B^{T}r_{s} = 0$ for all s, while the latter condition is equivalent to $C^{T}v_{s,s^{\prime}} + D(s,s^{\prime},x,\dot{x})^{T}q_{s,s^{\prime}} = 0$ for all $s,s^{\prime}$.
\end{proof}

We finally give an SOS program for verifying a CBF for (\ref{eq:Lagrangian-dynamics}).

\begin{theorem}
\label{theorem:Lagrangian-SOS}
The function $b$ is a CBF for the system with dynamics (\ref{eq:Lagrangian-dynamics}) if and only if there exist polynomials $\eta$, $\theta_{s}$, $\lambda_{s,s^{\prime}}$, and $\phi \in \Sigma[w_{s},v_{s,s^{\prime}},r_{s},q_{s,s^{\prime}}]$ such that 
\begin{multline*}
\eta b + \sum_{s}{\theta_{s}(A_{s}^{T}w_{s} + B^{T}r_{s})}\\ + \sum_{s,s^{\prime}}{\lambda_{s,s^{\prime}}(C^{T}v_{s,s^{\prime}} + D(s,s^{\prime},x,\dot{x})^{T}q_{s,s^{\prime}})} + \phi +1 = 0.
\end{multline*}
\end{theorem}

\begin{proof}
The proof follows from Lemma \ref{lemma:Lagrangian-outer-Farkas} and the Positivstellensatz.
\end{proof}

%\begin{proposition}
%\label{prop:Lagrangian-CBF-equivalent}
%The function $b(x,\dot{x})$ is a CBF if there do not exist $x,\dot{x},(w_{s,1},r_{s,1},w_{s,s^{\prime},2},r_{s,s^{\prime},2}$ for $s,s^{\prime} \in \mathcal{U}$  satisfying $b(x,\dot{x}) = 0$, $w_{s,1} \geq 0$, $w_{s,1} \neq 0$, $r_{1} \geq 0$, $A(s,x,\dot{x})^{T}w_{s,1} + B(x,\dot{x})^{T}r_{s,1} = 0$, $w_{s,s^{\prime},2} \geq 0$, $w_{s,s^{\prime},2} \neq 0$, and $C^{T}w_{s,s^{\prime},2} + D(s,s^{\prime},x,\dot{x})^{T}r = 0$.
%\end{proposition}
%
%\begin{proof}
%Follows from applying Lemma \ref{lemma:Lagrange-inner-Farkas} to the conditions of Lemma \ref{lemma:Lagrange-inner-Farkas}.
%\end{proof}

